Converting Binary Floating-Point Numbers to Shortest Decimal Strings: An Experimental Review

When sharing or logging numerical data, we must convert binary floating-point numbers into their decimal string representations. For example, the number $\pi$ might become 3.1415927. Engineers have perfected many algorithms for producing such accurate, short strings. We present an empirical comparison across diverse hardware architectures and datasets. Cutting-edge techniques like Schubfach and Dragonbox achieve up to a tenfold speedup over Steele and White's Dragon4, executing as few as 210 instructions per conversion compared to Dragon4's 1500-5000 instructions. Often per their specification, none of the implementations we surveyed consistently produced the shortest possible strings-some generate outputs up to 30% longer than optimal. We find that standard library implementations in languages such as C++ and Swift execute significantly more instructions than the fastest methods, with performance gaps varying across CPU architectures and compilers. We suggest some optimization targets for future research.

==> results/AMD_Ryzen9_9900X/Ryzen9900x_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 160 & 4500 & 5.1 \\ 
netlib & 540 & 11000 & 3.9 \\ 
fmt\_format & 35 & 840 & 4.4 \\ 
grisu3 & 28 & 600 & 3.8 \\ 
grisu\_exact & 22 & 480 & 3.8 \\ 
schubfach & 23 & 460 & 3.7 \\ 
dragonbox & 18 & 390 & 4.1 \\ 
ryu & 22 & 530 & 4.4 \\ 
teju\_jagua & 23 & 440 & 3.5 \\ 
double\_conversion & 50 & 1200 & 4.2 \\ 
swiftDtoa & 24 & 530 & 4.0 \\ 
yy\_double & 19 & 400 & 3.8 \\ 
std::to\_chars & 29 & 790 & 4.9 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 78 & 2400 & 5.6 \\ 
fmt\_format & 33 & 730 & 4.1 \\ 
grisu\_exact & 21 & 430 & 3.6 \\ 
schubfach & 18 & 400 & 4.0 \\ 
dragonbox & 17 & 340 & 3.8 \\ 
ryu & 20 & 450 & 4.2 \\ 
teju\_jagua & 21 & 410 & 3.5 \\ 
double\_conversion & 43 & 1000 & 4.3 \\ 
swiftDtoa & 20 & 470 & 4.2 \\ 
std::to\_chars & 25 & 630 & 4.6 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 76 & 2200 & 5.3 \\ 
netlib & 210 & 3900 & 3.5 \\ 
fmt\_format & 27 & 580 & 3.9 \\ 
grisu3 & 12 & 290 & 4.4 \\ 
grisu\_exact & 16 & 340 & 3.9 \\ 
schubfach & 9.9 & 240 & 4.4 \\ 
dragonbox & 12 & 250 & 3.7 \\ 
ryu & 13 & 320 & 4.3 \\ 
teju\_jagua & 11 & 240 & 3.9 \\ 
double\_conversion & 31 & 740 & 4.4 \\ 
swiftDtoa & 20 & 440 & 4.0 \\ 
yy\_double & 9.0 & 190 & 3.8 \\ 
std::to\_chars & 19 & 500 & 4.9 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 54 & 1600 & 5.6 \\ 
fmt\_format & 23 & 490 & 3.9 \\ 
grisu\_exact & 15 & 290 & 3.6 \\ 
schubfach & 9.8 & 220 & 4.0 \\ 
dragonbox & 10 & 210 & 3.6 \\ 
ryu & 16 & 380 & 4.2 \\ 
teju\_jagua & 12 & 230 & 3.6 \\ 
double\_conversion & 31 & 740 & 4.3 \\ 
swiftDtoa & 15 & 320 & 3.8 \\ 
std::to\_chars & 21 & 550 & 4.6 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 4700 & 5.2 \\ 
netlib & 580 & 12000 & 3.9 \\ 
fmt\_format & 30 & 530 & 3.2 \\ 
grisu3 & 25 & 470 & 3.3 \\ 
grisu\_exact & 19 & 320 & 3.0 \\ 
schubfach & 18 & 290 & 2.9 \\ 
dragonbox & 16 & 230 & 2.5 \\ 
ryu & 18 & 340 & 3.5 \\ 
teju\_jagua & 19 & 270 & 2.6 \\ 
double\_conversion & 44 & 980 & 4.0 \\ 
swiftDtoa & 23 & 380 & 3.0 \\ 
yy\_double & 13 & 230 & 3.2 \\ 
std::to\_chars & 25 & 600 & 4.3 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 81 & 2300 & 5.2 \\ 
fmt\_format & 24 & 420 & 3.2 \\ 
grisu\_exact & 19 & 260 & 2.5 \\ 
schubfach & 15 & 220 & 2.7 \\ 
dragonbox & 14 & 180 & 2.3 \\ 
ryu & 17 & 280 & 3.0 \\ 
teju\_jagua & 18 & 240 & 2.4 \\ 
double\_conversion & 38 & 820 & 3.9 \\ 
swiftDtoa & 21 & 320 & 2.7 \\ 
std::to\_chars & 23 & 460 & 3.6 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_all_none_native.tex <==
\begin{table}
  \centering
  \caption{Ryzen 9900X results (g++, 64-bit floats, native)}%
  \label{tab:ryzen9900xresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    schubfach & 9.8 & 250 & 4.6  & 24 & 490 & 3.7  & 19 & 320 & 3.0  \\
    dragonbox & 11 & 260 & 4.3  & 18 & 410 & 4.1  & 15 & 240 & 3.0  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_all_none_x86-64-v2.tex <==
\begin{table}
  \centering
  \caption{Ryzen 9900X results (g++, 64-bit floats, x86-64-v2)}%
  \label{tab:ryzen9900xresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    schubfach & 9.7 & 250 & 4.7  & 23 & 490 & 3.9  & 18 & 310 & 3.2  \\
    dragonbox & 11 & 260 & 4.2  & 18 & 410 & 4.1  & 15 & 240 & 2.9  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_all_none_x86-64-v3.tex <==
\begin{table}
  \centering
  \caption{Ryzen 9900X results (g++, 64-bit floats, x86-64-v3)}%
  \label{tab:ryzen9900xresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    schubfach & 9.6 & 250 & 4.7  & 23 & 480 & 3.8  & 19 & 310 & 2.9  \\
    dragonbox & 11 & 250 & 4.2  & 18 & 400 & 4.0  & 15 & 240 & 2.8  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_all_none_x86-64-v4.tex <==
\begin{table}
  \centering
  \caption{Ryzen 9900X results (g++, 64-bit floats, x86-64-v4)}%
  \label{tab:ryzen9900xresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    schubfach & 9.8 & 240 & 4.6  & 24 & 480 & 3.6  & 19 & 310 & 2.9  \\
    dragonbox & 11 & 260 & 4.2  & 18 & 410 & 4.1  & 15 & 250 & 3.0  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_all_none_x86-64.tex <==
\begin{table}
  \centering
  \caption{Ryzen 9900X results (g++, 64-bit floats, x86-64)}%
  \label{tab:ryzen9900xresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    schubfach & 9.8 & 250 & 4.6  & 23 & 490 & 3.9  & 18 & 310 & 3.2  \\
    dragonbox & 11 & 260 & 4.2  & 18 & 410 & 4.0  & 15 & 240 & 3.0  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 4700 & 5.2 \\ 
netlib & 550 & 11000 & 3.8 \\ 
fmt\_format & 40 & 840 & 3.8 \\ 
grisu3 & 29 & 630 & 4.0 \\ 
grisu\_exact & 24 & 520 & 3.9 \\ 
schubfach & 24 & 490 & 3.7 \\ 
dragonbox & 18 & 410 & 4.1 \\ 
ryu & 24 & 580 & 4.3 \\ 
teju\_jagua & 26 & 490 & 3.5 \\ 
double\_conversion & 45 & 1000 & 4.0 \\ 
swiftDtoa & 28 & 590 & 3.8 \\ 
yy\_double & 18 & 420 & 4.2 \\ 
std::to\_chars & 30 & 780 & 4.8 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_canada_none_native.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 24 & 490 & 3.7 \\ 
dragonbox & 18 & 410 & 4.1 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_canada_none_x86-64-v2.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 23 & 490 & 3.9 \\ 
dragonbox & 18 & 410 & 4.1 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_canada_none_x86-64-v3.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 23 & 480 & 3.8 \\ 
dragonbox & 18 & 400 & 4.0 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_canada_none_x86-64-v4.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 24 & 480 & 3.6 \\ 
dragonbox & 18 & 410 & 4.1 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_canada_none_x86-64.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 23 & 490 & 3.9 \\ 
dragonbox & 18 & 410 & 4.0 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 84 & 2400 & 5.3 \\ 
fmt\_format & 32 & 710 & 4.0 \\ 
grisu\_exact & 24 & 430 & 3.4 \\ 
schubfach & 18 & 410 & 4.0 \\ 
dragonbox & 18 & 340 & 3.5 \\ 
ryu & 20 & 480 & 4.3 \\ 
teju\_jagua & 21 & 410 & 3.5 \\ 
double\_conversion & 38 & 860 & 4.1 \\ 
swiftDtoa & 20 & 460 & 4.1 \\ 
std::to\_chars & 26 & 630 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 82 & 2300 & 5.0 \\ 
netlib & 210 & 3900 & 3.4 \\ 
fmt\_format & 30 & 570 & 3.5 \\ 
grisu3 & 12 & 290 & 4.5 \\ 
grisu\_exact & 18 & 370 & 3.7 \\ 
schubfach & 9.9 & 250 & 4.5 \\ 
dragonbox & 11 & 260 & 4.3 \\ 
ryu & 14 & 320 & 4.3 \\ 
teju\_jagua & 12 & 260 & 3.8 \\ 
double\_conversion & 27 & 610 & 4.0 \\ 
swiftDtoa & 23 & 490 & 3.8 \\ 
yy\_double & 9.6 & 200 & 3.8 \\ 
std::to\_chars & 18 & 490 & 4.8 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_mesh_none_native.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 9.8 & 250 & 4.6 \\ 
dragonbox & 11 & 260 & 4.3 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_mesh_none_x86-64-v2.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 9.7 & 250 & 4.7 \\ 
dragonbox & 11 & 260 & 4.2 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_mesh_none_x86-64-v3.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 9.6 & 250 & 4.7 \\ 
dragonbox & 11 & 250 & 4.2 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_mesh_none_x86-64-v4.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 9.8 & 240 & 4.6 \\ 
dragonbox & 11 & 260 & 4.2 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_mesh_none_x86-64.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 9.8 & 250 & 4.6 \\ 
dragonbox & 11 & 260 & 4.2 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 62 & 1700 & 5.0 \\ 
fmt\_format & 23 & 470 & 3.6 \\ 
grisu\_exact & 16 & 310 & 3.5 \\ 
schubfach & 9.8 & 210 & 3.9 \\ 
dragonbox & 10 & 200 & 3.6 \\ 
ryu & 16 & 390 & 4.3 \\ 
teju\_jagua & 12 & 230 & 3.6 \\ 
double\_conversion & 27 & 610 & 4.1 \\ 
swiftDtoa & 15 & 300 & 3.6 \\ 
std::to\_chars & 21 & 540 & 4.6 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 190 & 5000 & 4.9 \\ 
netlib & 580 & 12000 & 3.8 \\ 
fmt\_format & 35 & 560 & 2.9 \\ 
grisu3 & 26 & 510 & 3.6 \\ 
grisu\_exact & 21 & 370 & 3.1 \\ 
schubfach & 19 & 320 & 3.0 \\ 
dragonbox & 15 & 240 & 3.0 \\ 
ryu & 20 & 400 & 3.5 \\ 
teju\_jagua & 22 & 320 & 2.6 \\ 
double\_conversion & 39 & 810 & 3.7 \\ 
swiftDtoa & 27 & 440 & 3.0 \\ 
yy\_double & 15 & 250 & 3.0 \\ 
std::to\_chars & 25 & 600 & 4.3 \\ 
\bottomrule
\end{tabular}


==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_uniform_01_none_native.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 19 & 320 & 3.0 \\ 
dragonbox & 15 & 240 & 3.0 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_uniform_01_none_x86-64-v2.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 18 & 310 & 3.2 \\ 
dragonbox & 15 & 240 & 2.9 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_uniform_01_none_x86-64-v3.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 19 & 310 & 2.9 \\ 
dragonbox & 15 & 240 & 2.8 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_uniform_01_none_x86-64-v4.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 19 & 310 & 2.9 \\ 
dragonbox & 15 & 250 & 3.0 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_uniform_01_none_x86-64.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
schubfach & 18 & 310 & 3.2 \\ 
dragonbox & 15 & 240 & 3.0 \\ 
\bottomrule
\end{tabular}



==> results/AMD_Ryzen9_9900X/Ryzen9900x_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 99 & 2400 & 4.4 \\ 
fmt\_format & 25 & 410 & 3.0 \\ 
grisu\_exact & 19 & 270 & 2.5 \\ 
schubfach & 14 & 230 & 2.9 \\ 
dragonbox & 13 & 170 & 2.4 \\ 
ryu & 17 & 310 & 3.2 \\ 
teju\_jagua & 18 & 240 & 2.4 \\ 
double\_conversion & 34 & 660 & 3.6 \\ 
swiftDtoa & 21 & 300 & 2.6 \\ 
std::to\_chars & 23 & 450 & 3.6 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_canada_F6.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 80 & 1200 & 3.6 \\ 
netlib & 270 & 3700 & 3.2 \\ 
abseil & 37 & 800 & 5.1 \\ 
snprintf & 86 & 1400 & 3.8 \\ 
fmt\_format & 42 & 1000 & 5.8 \\ 
ryu & 16 & 450 & 6.3 \\ 
double\_conversion & 35 & 520 & 3.5 \\ 
std::to\_chars & 35 & 690 & 4.5 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_canada_F6s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 78 & 1100 & 3.2 \\ 
netlib & 230 & 3200 & 3.3 \\ 
abseil & 37 & 800 & 5.0 \\ 
snprintf & 84 & 1400 & 3.9 \\ 
fmt\_format & 43 & 1000 & 5.6 \\ 
double\_conversion & 35 & 520 & 3.4 \\ 
std::to\_chars & 35 & 700 & 4.5 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 150 & 3000 & 4.8 \\ 
netlib & 790 & 12000 & 3.5 \\ 
fmt\_format & 29 & 640 & 5.0 \\ 
grisu3 & 24 & 440 & 4.2 \\ 
grisu\_exact & 15 & 340 & 5.1 \\ 
schubfach & 12 & 310 & 5.9 \\ 
dragonbox & 9.5 & 240 & 5.6 \\ 
ryu & 12 & 330 & 6.3 \\ 
teju\_jagua & 15 & 280 & 4.2 \\ 
double\_conversion & 42 & 910 & 5.1 \\ 
swiftDtoa & 16 & 360 & 5.1 \\ 
yy\_double & 8.0 & 220 & 6.0 \\ 
std::to\_chars & 15 & 440 & 6.6 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 80 & 1600 & 4.6 \\ 
fmt\_format & 22 & 540 & 5.7 \\ 
grisu\_exact & 12 & 250 & 4.6 \\ 
schubfach & 9.2 & 240 & 5.9 \\ 
dragonbox & 8.9 & 180 & 4.6 \\ 
ryu & 10 & 250 & 5.3 \\ 
teju\_jagua & 12 & 230 & 4.4 \\ 
double\_conversion & 34 & 760 & 5.2 \\ 
swiftDtoa & 12 & 300 & 5.6 \\ 
std::to\_chars & 15 & 400 & 6.0 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_mesh_F6.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 46 & 900 & 4.4 \\ 
netlib & 160 & 2100 & 2.9 \\ 
abseil & 31 & 770 & 5.7 \\ 
snprintf & 71 & 1300 & 4.2 \\ 
fmt\_format & 33 & 910 & 6.3 \\ 
ryu & 12 & 380 & 6.9 \\ 
double\_conversion & 22 & 550 & 5.5 \\ 
std::to\_chars & 22 & 590 & 6.1 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_mesh_F6s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 44 & 830 & 4.3 \\ 
netlib & 150 & 2000 & 3.0 \\ 
abseil & 31 & 770 & 5.8 \\ 
snprintf & 71 & 1300 & 4.2 \\ 
fmt\_format & 34 & 910 & 6.1 \\ 
double\_conversion & 23 & 550 & 5.6 \\ 
std::to\_chars & 22 & 600 & 6.0 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 69 & 1500 & 5.3 \\ 
netlib & 280 & 4000 & 3.5 \\ 
fmt\_format & 22 & 530 & 5.4 \\ 
grisu3 & 10 & 260 & 5.6 \\ 
grisu\_exact & 11 & 320 & 6.3 \\ 
schubfach & 7.2 & 210 & 6.4 \\ 
dragonbox & 7.7 & 220 & 6.6 \\ 
ryu & 9.9 & 270 & 6.0 \\ 
teju\_jagua & 8.0 & 200 & 5.6 \\ 
double\_conversion & 26 & 640 & 5.5 \\ 
swiftDtoa & 14 & 390 & 6.0 \\ 
yy\_double & 4.9 & 160 & 7.1 \\ 
std::to\_chars & 13 & 350 & 5.8 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 53 & 1200 & 5.3 \\ 
fmt\_format & 18 & 450 & 5.7 \\ 
grisu\_exact & 8.4 & 240 & 6.4 \\ 
schubfach & 6.7 & 190 & 6.1 \\ 
dragonbox & 6.3 & 170 & 6.1 \\ 
ryu & 10 & 300 & 6.5 \\ 
teju\_jagua & 7.2 & 190 & 5.8 \\ 
double\_conversion & 28 & 640 & 5.2 \\ 
swiftDtoa & 11 & 290 & 5.7 \\ 
std::to\_chars & 15 & 420 & 6.4 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_uniform_01_F6.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 70 & 1100 & 3.6 \\ 
netlib & 260 & 3600 & 3.3 \\ 
abseil & 33 & 730 & 5.0 \\ 
snprintf & 86 & 1400 & 3.7 \\ 
fmt\_format & 38 & 870 & 5.4 \\ 
ryu & 14 & 280 & 4.6 \\ 
double\_conversion & 24 & 510 & 4.8 \\ 
std::to\_chars & 22 & 470 & 4.9 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_uniform_01_F6s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 64 & 970 & 3.5 \\ 
netlib & 210 & 3100 & 3.5 \\ 
abseil & 32 & 730 & 5.0 \\ 
snprintf & 84 & 1400 & 3.8 \\ 
fmt\_format & 38 & 870 & 5.3 \\ 
double\_conversion & 26 & 510 & 4.5 \\ 
std::to\_chars & 22 & 470 & 4.8 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 3300 & 4.6 \\ 
netlib & 830 & 13000 & 3.6 \\ 
fmt\_format & 30 & 510 & 3.8 \\ 
grisu3 & 26 & 470 & 4.0 \\ 
grisu\_exact & 18 & 340 & 4.2 \\ 
schubfach & 14 & 290 & 4.7 \\ 
dragonbox & 12 & 230 & 4.2 \\ 
ryu & 13 & 310 & 5.4 \\ 
teju\_jagua & 15 & 270 & 3.9 \\ 
double\_conversion & 43 & 880 & 4.8 \\ 
swiftDtoa & 20 & 390 & 4.4 \\ 
yy\_double & 7.4 & 210 & 6.2 \\ 
std::to\_chars & 16 & 410 & 5.6 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/Apple_M4_Max_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 88 & 1600 & 4.4 \\ 
fmt\_format & 20 & 410 & 4.5 \\ 
grisu\_exact & 15 & 250 & 3.6 \\ 
schubfach & 12 & 230 & 4.3 \\ 
dragonbox & 9.9 & 170 & 3.8 \\ 
ryu & 13 & 240 & 4.1 \\ 
teju\_jagua & 15 & 230 & 3.3 \\ 
double\_conversion & 34 & 730 & 5.0 \\ 
swiftDtoa & 19 & 320 & 3.8 \\ 
std::to\_chars & 19 & 390 & 4.6 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_bitcoin_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 100 & 2200 & 4.7 \\ 
netlib & 530 & 8500 & 3.6 \\ 
fmt\_format & 25 & 670 & 5.8 \\ 
grisu3 & 12 & 320 & 5.5 \\ 
grisu\_exact & 12 & 350 & 6.2 \\ 
schubfach & 8.4 & 310 & 7.4 \\ 
dragonboxlm & 7.7 & 250 & 6.5 \\ 
dragonbox & 8.6 & 270 & 6.4 \\ 
ryu & 13 & 420 & 6.6 \\ 
teju\_jagua & 9.0 & 260 & 5.8 \\ 
double\_conversion & 32 & 800 & 5.4 \\ 
swiftDtoa & 13 & 370 & 6.0 \\ 
yy\_double & 7.7 & 230 & 6.1 \\ 
std::to\_chars & 17 & 540 & 6.7 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_bitcoin_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 69 & 1600 & 5.0 \\ 
fmt\_format & 20 & 550 & 5.8 \\ 
grisu\_exact & 7.5 & 270 & 7.2 \\ 
schubfach & 7.9 & 260 & 6.7 \\ 
dragonboxlm & 5.7 & 190 & 6.3 \\ 
dragonbox & 6.4 & 200 & 5.9 \\ 
ryu & 7.9 & 270 & 6.8 \\ 
teju\_jagua & 5.1 & 200 & 7.7 \\ 
double\_conversion & 44 & 810 & 4.0 \\ 
swiftDtoa & 11 & 320 & 6.0 \\ 
std::to\_chars & 14 & 430 & 6.5 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_gaia_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 3200 & 4.4 \\ 
netlib & 830 & 12000 & 3.5 \\ 
fmt\_format & 37 & 630 & 4.1 \\ 
grisu3 & 29 & 460 & 3.8 \\ 
grisu\_exact & 23 & 340 & 3.6 \\ 
schubfach & 16 & 310 & 4.8 \\ 
dragonboxlm & 14 & 210 & 3.6 \\ 
dragonbox & 14 & 250 & 4.1 \\ 
ryu & 16 & 320 & 4.8 \\ 
teju\_jagua & 16 & 210 & 3.0 \\ 
double\_conversion & 50 & 940 & 4.5 \\ 
swiftDtoa & 20 & 370 & 4.3 \\ 
yy\_double & 8.6 & 220 & 6.0 \\ 
std::to\_chars & 21 & 430 & 5.0 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_gaia_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 90 & 1600 & 4.3 \\ 
fmt\_format & 28 & 520 & 4.4 \\ 
grisu\_exact & 18 & 250 & 3.3 \\ 
schubfach & 12 & 250 & 4.9 \\ 
dragonboxlm & 13 & 170 & 3.1 \\ 
dragonbox & 12 & 180 & 3.5 \\ 
ryu & 14 & 250 & 4.3 \\ 
teju\_jagua & 17 & 180 & 2.6 \\ 
double\_conversion & 41 & 770 & 4.4 \\ 
swiftDtoa & 18 & 300 & 4.1 \\ 
std::to\_chars & 19 & 400 & 4.9 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_marine_ik_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 60 & 1400 & 5.6 \\ 
netlib & 350 & 5200 & 3.4 \\ 
fmt\_format & 18 & 500 & 6.2 \\ 
grisu3 & 11 & 290 & 5.8 \\ 
grisu\_exact & 11 & 320 & 6.4 \\ 
schubfach & 7.3 & 260 & 7.8 \\ 
dragonboxlm & 6.4 & 210 & 7.2 \\ 
dragonbox & 6.6 & 220 & 7.3 \\ 
ryu & 17 & 450 & 5.9 \\ 
teju\_jagua & 11 & 250 & 5.0 \\ 
double\_conversion & 25 & 650 & 5.9 \\ 
swiftDtoa & 16 & 400 & 5.6 \\ 
yy\_double & 7.8 & 220 & 6.2 \\ 
std::to\_chars & 18 & 540 & 6.7 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_marine_ik_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 55 & 1400 & 5.9 \\ 
fmt\_format & 14 & 430 & 6.9 \\ 
grisu\_exact & 7.9 & 260 & 7.2 \\ 
schubfach & 6.3 & 230 & 8.2 \\ 
dragonboxlm & 5.6 & 170 & 6.9 \\ 
dragonbox & 5.7 & 180 & 7.1 \\ 
ryu & 8.2 & 270 & 7.2 \\ 
teju\_jagua & 7.0 & 190 & 6.1 \\ 
double\_conversion & 26 & 690 & 5.9 \\ 
swiftDtoa & 10 & 310 & 6.6 \\ 
std::to\_chars & 13 & 410 & 7.0 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_mobilenetv3_large_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 100 & 1900 & 4.6 \\ 
netlib & 470 & 6600 & 3.4 \\ 
fmt\_format & 31 & 510 & 4.0 \\ 
grisu3 & 24 & 340 & 3.4 \\ 
grisu\_exact & 23 & 340 & 3.6 \\ 
schubfach & 11 & 260 & 5.8 \\ 
dragonboxlm & 14 & 210 & 3.6 \\ 
dragonbox & 14 & 220 & 3.9 \\ 
ryu & 25 & 420 & 3.9 \\ 
teju\_jagua & 20 & 240 & 2.9 \\ 
double\_conversion & 40 & 700 & 4.3 \\ 
swiftDtoa & 21 & 350 & 3.9 \\ 
yy\_double & 8.6 & 220 & 6.1 \\ 
std::to\_chars & 32 & 520 & 3.8 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_mobilenetv3_large_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 100 & 2000 & 4.6 \\ 
fmt\_format & 28 & 430 & 3.7 \\ 
grisu\_exact & 21 & 260 & 2.9 \\ 
schubfach & 13 & 240 & 4.4 \\ 
dragonboxlm & 13 & 170 & 3.2 \\ 
dragonbox & 14 & 180 & 3.1 \\ 
ryu & 14 & 250 & 4.3 \\ 
teju\_jagua & 17 & 190 & 2.6 \\ 
double\_conversion & 42 & 750 & 4.3 \\ 
swiftDtoa & 21 & 330 & 3.8 \\ 
std::to\_chars & 22 & 400 & 4.3 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_noaa_gfs_1p00_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 71 & 1500 & 5.0 \\ 
netlib & 360 & 5100 & 3.4 \\ 
fmt\_format & 26 & 530 & 5.1 \\ 
grisu3 & 15 & 270 & 4.2 \\ 
grisu\_exact & 17 & 320 & 4.5 \\ 
schubfach & 8.9 & 230 & 6.1 \\ 
dragonboxlm & 9.6 & 180 & 4.6 \\ 
dragonbox & 9.3 & 190 & 4.9 \\ 
ryu & 17 & 360 & 5.0 \\ 
teju\_jagua & 15 & 230 & 3.6 \\ 
double\_conversion & 32 & 610 & 4.7 \\ 
swiftDtoa & 15 & 290 & 4.5 \\ 
yy\_double & 7.8 & 200 & 6.1 \\ 
std::to\_chars & 22 & 460 & 5.0 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_noaa_gfs_1p00_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 67 & 1400 & 5.0 \\ 
fmt\_format & 22 & 470 & 5.2 \\ 
grisu\_exact & 14 & 240 & 4.0 \\ 
schubfach & 9.0 & 210 & 5.5 \\ 
dragonboxlm & 9.1 & 150 & 4.0 \\ 
dragonbox & 9.1 & 160 & 4.2 \\ 
ryu & 11 & 220 & 5.0 \\ 
teju\_jagua & 12 & 190 & 3.7 \\ 
double\_conversion & 35 & 660 & 4.6 \\ 
swiftDtoa & 13 & 260 & 4.7 \\ 
std::to\_chars & 16 & 350 & 5.3 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_noaa_global_hourly_2023_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 36 & 890 & 6.0 \\ 
netlib & 190 & 2600 & 3.4 \\ 
fmt\_format & 27 & 560 & 4.9 \\ 
grisu3 & 11 & 260 & 5.6 \\ 
grisu\_exact & 13 & 300 & 5.3 \\ 
schubfach & 7.9 & 220 & 6.3 \\ 
dragonboxlm & 8.4 & 200 & 5.5 \\ 
dragonbox & 8.6 & 200 & 5.4 \\ 
ryu & 14 & 340 & 5.6 \\ 
teju\_jagua & 9.2 & 200 & 5.1 \\ 
double\_conversion & 26 & 560 & 5.2 \\ 
swiftDtoa & 16 & 390 & 5.9 \\ 
yy\_double & 6.4 & 170 & 6.5 \\ 
std::to\_chars & 17 & 440 & 5.9 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_noaa_global_hourly_2023_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 34 & 840 & 6.0 \\ 
fmt\_format & 22 & 500 & 5.5 \\ 
grisu\_exact & 10 & 230 & 5.2 \\ 
schubfach & 6.8 & 190 & 6.6 \\ 
dragonboxlm & 7.4 & 170 & 5.4 \\ 
dragonbox & 7.7 & 170 & 5.1 \\ 
ryu & 13 & 310 & 5.6 \\ 
teju\_jagua & 7.3 & 170 & 5.4 \\ 
double\_conversion & 27 & 610 & 5.5 \\ 
swiftDtoa & 11 & 260 & 5.8 \\ 
std::to\_chars & 18 & 440 & 5.9 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 3300 & 4.6 \\ 
netlib & 830 & 13000 & 3.6 \\ 
fmt\_format & 30 & 510 & 3.8 \\ 
grisu3 & 26 & 470 & 4.0 \\ 
grisu\_exact & 18 & 340 & 4.2 \\ 
schubfach & 14 & 290 & 4.7 \\ 
dragonbox & 12 & 230 & 4.2 \\ 
ryu & 13 & 310 & 5.4 \\ 
teju\_jagua & 15 & 270 & 3.9 \\ 
double\_conversion & 43 & 880 & 4.8 \\ 
swiftDtoa & 20 & 390 & 4.4 \\ 
yy\_double & 7.4 & 210 & 6.2 \\ 
std::to\_chars & 16 & 410 & 5.6 \\ 
\bottomrule
\end{tabular}


==> results/apple_m4/extra_datasets/Apple_M4_Max_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 88 & 1600 & 4.4 \\ 
fmt\_format & 20 & 410 & 4.5 \\ 
grisu\_exact & 15 & 250 & 3.6 \\ 
schubfach & 12 & 230 & 4.3 \\ 
dragonbox & 9.9 & 170 & 3.8 \\ 
ryu & 13 & 240 & 4.1 \\ 
teju\_jagua & 15 & 230 & 3.3 \\ 
double\_conversion & 34 & 730 & 5.0 \\ 
swiftDtoa & 19 & 320 & 3.8 \\ 
std::to\_chars & 19 & 390 & 4.6 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 340 & 4000 & 3.6 \\ 
netlib & 1300 & 12000 & 2.8 \\ 
fmt\_format & 94 & 830 & 2.8 \\ 
grisu3 & 70 & 620 & 2.8 \\ 
grisu\_exact & 57 & 510 & 2.8 \\ 
schubfach & 53 & 490 & 2.9 \\ 
dragonbox & 51 & 420 & 2.6 \\ 
ryu & 51 & 550 & 3.4 \\ 
teju\_jagua & 51 & 460 & 2.8 \\ 
double\_conversion & 130 & 1200 & 2.7 \\ 
swiftDtoa & 56 & 550 & 3.0 \\ 
yy\_double & 49 & 440 & 2.7 \\ 
std::to\_chars & 77 & 850 & 3.4 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 190 & 2100 & 3.4 \\ 
fmt\_format & 77 & 740 & 3.0 \\ 
grisu\_exact & 48 & 460 & 2.9 \\ 
schubfach & 43 & 430 & 3.0 \\ 
dragonbox & 44 & 370 & 2.6 \\ 
ryu & 45 & 480 & 3.3 \\ 
teju\_jagua & 49 & 430 & 2.7 \\ 
double\_conversion & 120 & 1000 & 2.7 \\ 
swiftDtoa & 47 & 490 & 3.2 \\ 
std::to\_chars & 69 & 670 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 1900 & 3.5 \\ 
netlib & 450 & 3900 & 2.7 \\ 
fmt\_format & 61 & 540 & 2.7 \\ 
grisu3 & 28 & 290 & 3.1 \\ 
grisu\_exact & 34 & 340 & 3.1 \\ 
schubfach & 23 & 240 & 3.1 \\ 
dragonbox & 27 & 250 & 2.9 \\ 
ryu & 31 & 310 & 3.1 \\ 
teju\_jagua & 25 & 230 & 2.9 \\ 
double\_conversion & 78 & 710 & 2.8 \\ 
swiftDtoa & 42 & 440 & 3.2 \\ 
yy\_double & 24 & 200 & 2.5 \\ 
std::to\_chars & 52 & 510 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 1500 & 3.4 \\ 
fmt\_format & 51 & 460 & 2.8 \\ 
grisu\_exact & 30 & 300 & 3.0 \\ 
schubfach & 23 & 220 & 2.8 \\ 
dragonbox & 21 & 200 & 3.0 \\ 
ryu & 35 & 380 & 3.3 \\ 
teju\_jagua & 25 & 230 & 2.8 \\ 
double\_conversion & 78 & 720 & 2.8 \\ 
swiftDtoa & 32 & 310 & 3.0 \\ 
std::to\_chars & 56 & 550 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 370 & 4200 & 3.5 \\ 
netlib & 1300 & 12000 & 2.9 \\ 
fmt\_format & 61 & 500 & 2.6 \\ 
grisu3 & 61 & 470 & 2.4 \\ 
grisu\_exact & 38 & 320 & 2.6 \\ 
schubfach & 36 & 290 & 2.4 \\ 
dragonbox & 29 & 230 & 2.4 \\ 
ryu & 39 & 350 & 2.7 \\ 
teju\_jagua & 36 & 260 & 2.2 \\ 
double\_conversion & 110 & 970 & 2.7 \\ 
swiftDtoa & 45 & 370 & 2.5 \\ 
yy\_double & 32 & 240 & 2.3 \\ 
std::to\_chars & 60 & 640 & 3.3 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 190 & 2000 & 3.2 \\ 
fmt\_format & 48 & 390 & 2.5 \\ 
grisu\_exact & 36 & 270 & 2.3 \\ 
schubfach & 33 & 220 & 2.1 \\ 
dragonbox & 24 & 170 & 2.2 \\ 
ryu & 34 & 290 & 2.6 \\ 
teju\_jagua & 35 & 240 & 2.1 \\ 
double\_conversion & 93 & 790 & 2.6 \\ 
swiftDtoa & 40 & 310 & 2.4 \\ 
std::to\_chars & 58 & 460 & 2.4 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 370 & 4600 & 3.9 \\ 
netlib & 1300 & 12000 & 2.8 \\ 
fmt\_format & 130 & 1100 & 2.7 \\ 
grisu3 & 72 & 680 & 2.9 \\ 
grisu\_exact & 58 & 570 & 3.1 \\ 
schubfach & 64 & 550 & 2.7 \\ 
dragonbox & 49 & 450 & 2.8 \\ 
ryu & 58 & 630 & 3.3 \\ 
teju\_jagua & 60 & 520 & 2.7 \\ 
double\_conversion & 120 & 1100 & 2.6 \\ 
swiftDtoa & 74 & 660 & 2.7 \\ 
yy\_double & 52 & 490 & 2.9 \\ 
std::to\_chars & 80 & 860 & 3.3 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 200 & 2400 & 3.8 \\ 
fmt\_format & 110 & 890 & 2.6 \\ 
grisu\_exact & 56 & 480 & 2.7 \\ 
schubfach & 50 & 460 & 2.8 \\ 
dragonbox & 47 & 380 & 2.5 \\ 
ryu & 54 & 520 & 2.9 \\ 
teju\_jagua & 53 & 450 & 2.6 \\ 
double\_conversion & 100 & 910 & 2.7 \\ 
swiftDtoa & 54 & 490 & 2.8 \\ 
std::to\_chars & 76 & 680 & 2.8 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 2300 & 4.0 \\ 
netlib & 460 & 3900 & 2.6 \\ 
fmt\_format & 63 & 610 & 3.0 \\ 
grisu3 & 31 & 310 & 3.0 \\ 
grisu\_exact & 38 & 390 & 3.1 \\ 
schubfach & 27 & 270 & 3.0 \\ 
dragonbox & 24 & 270 & 3.4 \\ 
ryu & 33 & 350 & 3.2 \\ 
teju\_jagua & 27 & 260 & 3.0 \\ 
double\_conversion & 69 & 630 & 2.8 \\ 
swiftDtoa & 56 & 530 & 2.9 \\ 
yy\_double & 29 & 230 & 2.5 \\ 
std::to\_chars & 54 & 520 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 140 & 1700 & 3.8 \\ 
fmt\_format & 56 & 530 & 2.9 \\ 
grisu\_exact & 35 & 330 & 2.8 \\ 
schubfach & 24 & 230 & 3.0 \\ 
dragonbox & 22 & 210 & 3.0 \\ 
ryu & 35 & 400 & 3.5 \\ 
teju\_jagua & 26 & 240 & 2.9 \\ 
double\_conversion & 70 & 640 & 2.8 \\ 
swiftDtoa & 34 & 310 & 2.8 \\ 
std::to\_chars & 58 & 560 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 370 & 4900 & 4.0 \\ 
netlib & 1300 & 12000 & 2.9 \\ 
fmt\_format & 67 & 590 & 2.7 \\ 
grisu3 & 61 & 520 & 2.6 \\ 
grisu\_exact & 41 & 380 & 2.8 \\ 
schubfach & 41 & 340 & 2.6 \\ 
dragonbox & 30 & 250 & 2.6 \\ 
ryu & 40 & 410 & 3.2 \\ 
teju\_jagua & 39 & 320 & 2.5 \\ 
double\_conversion & 99 & 830 & 2.6 \\ 
swiftDtoa & 59 & 460 & 2.4 \\ 
yy\_double & 41 & 290 & 2.1 \\ 
std::to\_chars & 60 & 640 & 3.3 \\ 
\bottomrule
\end{tabular}


==> results/c5a.24xlarge/AMD_EPYC_7R32_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 190 & 2400 & 3.8 \\ 
fmt\_format & 56 & 460 & 2.5 \\ 
grisu\_exact & 40 & 290 & 2.2 \\ 
schubfach & 31 & 250 & 2.5 \\ 
dragonbox & 24 & 180 & 2.3 \\ 
ryu & 34 & 320 & 2.8 \\ 
teju\_jagua & 34 & 240 & 2.2 \\ 
double\_conversion & 77 & 690 & 2.8 \\ 
swiftDtoa & 39 & 290 & 2.3 \\ 
std::to\_chars & 57 & 460 & 2.5 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_clang++_all_none.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8124M results (clang++, 64-bit floats)}%
  \label{tab:intelrxeonrplatinum8124mcpu300ghzresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 200 & 2100 & 3.0  & 440 & 4400 & 2.9  & 460 & 4600 & 2.9  \\
    fmt\_format & 53 & 530 & 2.9  & 79 & 840 & 3.0  & 56 & 500 & 2.6  \\
    grisu3 & 28 & 290 & 2.9  & 68 & 630 & 2.6  & 55 & 470 & 2.5  \\
    grisu\_exact & 33 & 340 & 3.0  & 51 & 510 & 2.9  & 37 & 320 & 2.5  \\
    schubfach & 22 & 240 & 3.1  & 53 & 500 & 2.7  & 35 & 290 & 2.4  \\
    dragonbox & 26 & 250 & 2.7  & 43 & 420 & 2.8  & 29 & 220 & 2.2  \\
    ryu & 29 & 310 & 3.0  & 50 & 550 & 3.1  & 34 & 330 & 2.8  \\
    double\_conversion & 84 & 720 & 2.4  & 150 & 1200 & 2.3  & 110 & 960 & 2.4  \\
    swiftDtoa & 38 & 420 & 3.2  & 55 & 540 & 2.8  & 42 & 360 & 2.5  \\
    std::to\_chars & 48 & 510 & 3.0  & 80 & 850 & 3.1  & 63 & 640 & 2.9  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_clang++_all_s.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8124M results (clang++, 32-bit floats)}%
  \label{tab:intelrxeonrplatinum8124mcpu300ghzresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 160 & 1600 & 2.9  & 240 & 2300 & 2.8  & 240 & 2200 & 2.6  \\
    fmt\_format & 48 & 460 & 2.8  & 72 & 730 & 2.9  & 47 & 390 & 2.4  \\
    grisu\_exact & 29 & 300 & 3.0  & 50 & 460 & 2.6  & 35 & 270 & 2.2  \\
    schubfach & 20 & 220 & 3.1  & 43 & 430 & 2.9  & 28 & 230 & 2.4  \\
    dragonbox & 20 & 200 & 2.9  & 41 & 370 & 2.6  & 23 & 170 & 2.2  \\
    ryu & 32 & 380 & 3.4  & 49 & 480 & 2.9  & 31 & 290 & 2.7  \\
    double\_conversion & 84 & 730 & 2.5  & 130 & 1000 & 2.3  & 92 & 800 & 2.5  \\
    swiftDtoa & 29 & 310 & 3.0  & 48 & 490 & 2.9  & 36 & 310 & 2.4  \\
    std::to\_chars & 51 & 550 & 3.1  & 68 & 670 & 2.8  & 51 & 460 & 2.6  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 440 & 4400 & 2.9 \\ 
netlib & 1500 & 12000 & 2.2 \\ 
fmt\_format & 79 & 840 & 3.0 \\ 
grisu3 & 68 & 630 & 2.6 \\ 
grisu\_exact & 51 & 510 & 2.9 \\ 
schubfach & 53 & 500 & 2.7 \\ 
dragonbox & 43 & 420 & 2.8 \\ 
ryu & 50 & 550 & 3.1 \\ 
teju\_jagua & 54 & 470 & 2.5 \\ 
double\_conversion & 150 & 1200 & 2.3 \\ 
swiftDtoa & 55 & 540 & 2.8 \\ 
yy\_double & 42 & 430 & 2.9 \\ 
std::to\_chars & 80 & 850 & 3.1 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 240 & 2300 & 2.8 \\ 
fmt\_format & 72 & 730 & 2.9 \\ 
grisu\_exact & 50 & 460 & 2.6 \\ 
schubfach & 43 & 430 & 2.9 \\ 
dragonbox & 41 & 370 & 2.6 \\ 
ryu & 49 & 480 & 2.9 \\ 
teju\_jagua & 49 & 440 & 2.6 \\ 
double\_conversion & 130 & 1000 & 2.3 \\ 
swiftDtoa & 48 & 490 & 2.9 \\ 
std::to\_chars & 68 & 670 & 2.8 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 200 & 2100 & 3.0 \\ 
netlib & 520 & 3900 & 2.1 \\ 
fmt\_format & 53 & 530 & 2.9 \\ 
grisu3 & 28 & 290 & 2.9 \\ 
grisu\_exact & 33 & 340 & 3.0 \\ 
schubfach & 22 & 240 & 3.1 \\ 
dragonbox & 26 & 250 & 2.7 \\ 
ryu & 29 & 310 & 3.0 \\ 
teju\_jagua & 25 & 240 & 2.7 \\ 
double\_conversion & 84 & 720 & 2.4 \\ 
swiftDtoa & 38 & 420 & 3.2 \\ 
yy\_double & 18 & 190 & 3.0 \\ 
std::to\_chars & 48 & 510 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 160 & 1600 & 2.9 \\ 
fmt\_format & 48 & 460 & 2.8 \\ 
grisu\_exact & 29 & 300 & 3.0 \\ 
schubfach & 20 & 220 & 3.1 \\ 
dragonbox & 20 & 200 & 2.9 \\ 
ryu & 32 & 380 & 3.4 \\ 
teju\_jagua & 24 & 230 & 2.8 \\ 
double\_conversion & 84 & 730 & 2.5 \\ 
swiftDtoa & 29 & 310 & 3.0 \\ 
std::to\_chars & 51 & 550 & 3.1 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 460 & 4600 & 2.9 \\ 
netlib & 1600 & 12000 & 2.2 \\ 
fmt\_format & 56 & 500 & 2.6 \\ 
grisu3 & 55 & 470 & 2.5 \\ 
grisu\_exact & 37 & 320 & 2.5 \\ 
schubfach & 35 & 290 & 2.4 \\ 
dragonbox & 29 & 220 & 2.2 \\ 
ryu & 34 & 330 & 2.8 \\ 
teju\_jagua & 36 & 270 & 2.1 \\ 
double\_conversion & 110 & 960 & 2.4 \\ 
swiftDtoa & 42 & 360 & 2.5 \\ 
yy\_double & 25 & 240 & 2.7 \\ 
std::to\_chars & 63 & 640 & 2.9 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 240 & 2200 & 2.6 \\ 
fmt\_format & 47 & 390 & 2.4 \\ 
grisu\_exact & 35 & 270 & 2.2 \\ 
schubfach & 28 & 230 & 2.4 \\ 
dragonbox & 23 & 170 & 2.2 \\ 
ryu & 31 & 290 & 2.7 \\ 
teju\_jagua & 33 & 240 & 2.1 \\ 
double\_conversion & 92 & 800 & 2.5 \\ 
swiftDtoa & 36 & 310 & 2.4 \\ 
std::to\_chars & 51 & 460 & 2.6 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_g++_all_none.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8124M results (g++, 64-bit floats)}%
  \label{tab:intelrxeonrplatinum8124mcpu300ghzresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 200 & 2200 & 3.3  & 420 & 4600 & 3.1  & 440 & 4900 & 3.2  \\
    fmt\_format & 61 & 610 & 2.9  & 110 & 1200 & 3.0  & 65 & 590 & 2.6  \\
    grisu3 & 30 & 310 & 2.9  & 69 & 680 & 2.8  & 53 & 520 & 2.8  \\
    grisu\_exact & 37 & 390 & 3.0  & 57 & 570 & 2.9  & 41 & 380 & 2.6  \\
    schubfach & 25 & 270 & 3.1  & 57 & 550 & 2.8  & 37 & 340 & 2.6  \\
    dragonbox & 26 & 270 & 2.9  & 45 & 450 & 2.9  & 29 & 250 & 2.4  \\
    ryu & 31 & 350 & 3.2  & 59 & 620 & 3.0  & 38 & 400 & 3.1  \\
    double\_conversion & 75 & 630 & 2.4  & 140 & 1000 & 2.2  & 100 & 830 & 2.4  \\
    swiftDtoa & 47 & 520 & 3.2  & 67 & 650 & 2.8  & 50 & 460 & 2.7  \\
    std::to\_chars & 48 & 510 & 3.0  & 81 & 860 & 3.0  & 62 & 640 & 3.0  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_g++_all_s.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8124M results (g++, 32-bit floats)}%
  \label{tab:intelrxeonrplatinum8124mcpu300ghzresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 160 & 1700 & 3.1  & 230 & 2400 & 3.0  & 230 & 2300 & 2.9  \\
    fmt\_format & 52 & 530 & 2.9  & 92 & 890 & 2.8  & 51 & 460 & 2.6  \\
    grisu\_exact & 34 & 330 & 2.8  & 52 & 480 & 2.7  & 37 & 290 & 2.2  \\
    schubfach & 22 & 230 & 3.0  & 46 & 450 & 2.8  & 30 & 250 & 2.4  \\
    dragonbox & 21 & 210 & 2.9  & 41 & 380 & 2.7  & 23 & 180 & 2.2  \\
    ryu & 34 & 400 & 3.3  & 49 & 520 & 3.0  & 33 & 320 & 2.8  \\
    double\_conversion & 77 & 640 & 2.4  & 120 & 910 & 2.2  & 82 & 680 & 2.4  \\
    swiftDtoa & 30 & 300 & 3.0  & 49 & 490 & 2.9  & 37 & 290 & 2.3  \\
    std::to\_chars & 55 & 560 & 2.9  & 69 & 680 & 2.8  & 52 & 460 & 2.6  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 420 & 4600 & 3.1 \\ 
netlib & 1500 & 12000 & 2.2 \\ 
fmt\_format & 110 & 1200 & 3.0 \\ 
grisu3 & 69 & 680 & 2.8 \\ 
grisu\_exact & 57 & 570 & 2.9 \\ 
schubfach & 57 & 550 & 2.8 \\ 
dragonbox & 45 & 450 & 2.9 \\ 
ryu & 59 & 620 & 3.0 \\ 
teju\_jagua & 58 & 520 & 2.6 \\ 
double\_conversion & 140 & 1000 & 2.2 \\ 
swiftDtoa & 67 & 650 & 2.8 \\ 
yy\_double & 47 & 490 & 3.0 \\ 
std::to\_chars & 81 & 860 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 230 & 2400 & 3.0 \\ 
fmt\_format & 92 & 890 & 2.8 \\ 
grisu\_exact & 52 & 480 & 2.7 \\ 
schubfach & 46 & 450 & 2.8 \\ 
dragonbox & 41 & 380 & 2.7 \\ 
ryu & 49 & 520 & 3.0 \\ 
teju\_jagua & 50 & 450 & 2.6 \\ 
double\_conversion & 120 & 910 & 2.2 \\ 
swiftDtoa & 49 & 490 & 2.9 \\ 
std::to\_chars & 69 & 680 & 2.8 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 200 & 2200 & 3.3 \\ 
netlib & 530 & 3900 & 2.2 \\ 
fmt\_format & 61 & 610 & 2.9 \\ 
grisu3 & 30 & 310 & 2.9 \\ 
grisu\_exact & 37 & 390 & 3.0 \\ 
schubfach & 25 & 270 & 3.1 \\ 
dragonbox & 26 & 270 & 2.9 \\ 
ryu & 31 & 350 & 3.2 \\ 
teju\_jagua & 26 & 260 & 2.8 \\ 
double\_conversion & 75 & 630 & 2.4 \\ 
swiftDtoa & 47 & 520 & 3.2 \\ 
yy\_double & 22 & 230 & 3.0 \\ 
std::to\_chars & 48 & 510 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 160 & 1700 & 3.1 \\ 
fmt\_format & 52 & 530 & 2.9 \\ 
grisu\_exact & 34 & 330 & 2.8 \\ 
schubfach & 22 & 230 & 3.0 \\ 
dragonbox & 21 & 210 & 2.9 \\ 
ryu & 34 & 400 & 3.3 \\ 
teju\_jagua & 24 & 240 & 2.9 \\ 
double\_conversion & 77 & 640 & 2.4 \\ 
swiftDtoa & 30 & 300 & 3.0 \\ 
std::to\_chars & 55 & 560 & 2.9 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 440 & 4900 & 3.2 \\ 
netlib & 1600 & 12000 & 2.2 \\ 
fmt\_format & 65 & 590 & 2.6 \\ 
grisu3 & 53 & 520 & 2.8 \\ 
grisu\_exact & 41 & 380 & 2.6 \\ 
schubfach & 37 & 340 & 2.6 \\ 
dragonbox & 29 & 250 & 2.4 \\ 
ryu & 38 & 400 & 3.1 \\ 
teju\_jagua & 38 & 320 & 2.4 \\ 
double\_conversion & 100 & 830 & 2.4 \\ 
swiftDtoa & 50 & 460 & 2.7 \\ 
yy\_double & 32 & 280 & 2.6 \\ 
std::to\_chars & 62 & 640 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c5n.metal/Intel_R__Xeon_R__Platinum_8124M_CPU__3.00GHz_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 230 & 2300 & 2.9 \\ 
fmt\_format & 51 & 460 & 2.6 \\ 
grisu\_exact & 37 & 290 & 2.2 \\ 
schubfach & 30 & 250 & 2.4 \\ 
dragonbox & 23 & 180 & 2.2 \\ 
ryu & 33 & 320 & 2.8 \\ 
teju\_jagua & 33 & 240 & 2.1 \\ 
double\_conversion & 82 & 680 & 2.4 \\ 
swiftDtoa & 37 & 290 & 2.3 \\ 
std::to\_chars & 52 & 460 & 2.6 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 270 & 4400 & 4.4 \\ 
netlib & 1200 & 12000 & 2.7 \\ 
fmt\_format & 67 & 840 & 3.4 \\ 
grisu3 & 53 & 630 & 3.2 \\ 
grisu\_exact & 41 & 510 & 3.4 \\ 
schubfach & 43 & 490 & 3.1 \\ 
dragonbox & 33 & 420 & 3.5 \\ 
ryu & 40 & 550 & 3.8 \\ 
teju\_jagua & 41 & 460 & 3.0 \\ 
double\_conversion & 100 & 1200 & 3.1 \\ 
swiftDtoa & 44 & 550 & 3.4 \\ 
yy\_double & 39 & 440 & 3.1 \\ 
std::to\_chars & 57 & 850 & 4.0 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 140 & 2300 & 4.4 \\ 
fmt\_format & 58 & 730 & 3.4 \\ 
grisu\_exact & 36 & 460 & 3.4 \\ 
schubfach & 37 & 430 & 3.2 \\ 
dragonbox & 31 & 370 & 3.2 \\ 
ryu & 36 & 480 & 3.6 \\ 
teju\_jagua & 36 & 430 & 3.2 \\ 
double\_conversion & 87 & 1000 & 3.2 \\ 
swiftDtoa & 37 & 490 & 3.5 \\ 
std::to\_chars & 50 & 670 & 3.6 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 120 & 2100 & 4.6 \\ 
netlib & 420 & 3900 & 2.5 \\ 
fmt\_format & 45 & 540 & 3.2 \\ 
grisu3 & 22 & 290 & 3.5 \\ 
grisu\_exact & 26 & 340 & 3.5 \\ 
schubfach & 18 & 240 & 3.5 \\ 
dragonbox & 20 & 250 & 3.3 \\ 
ryu & 23 & 310 & 3.6 \\ 
teju\_jagua & 20 & 230 & 3.1 \\ 
double\_conversion & 58 & 720 & 3.3 \\ 
swiftDtoa & 34 & 440 & 3.4 \\ 
yy\_double & 19 & 200 & 2.8 \\ 
std::to\_chars & 36 & 510 & 3.8 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 94 & 1600 & 4.5 \\ 
fmt\_format & 39 & 460 & 3.2 \\ 
grisu\_exact & 23 & 300 & 3.4 \\ 
schubfach & 18 & 220 & 3.3 \\ 
dragonbox & 16 & 200 & 3.3 \\ 
ryu & 28 & 380 & 3.6 \\ 
teju\_jagua & 20 & 230 & 3.1 \\ 
double\_conversion & 60 & 730 & 3.2 \\ 
swiftDtoa & 25 & 310 & 3.4 \\ 
std::to\_chars & 40 & 550 & 3.7 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 270 & 4600 & 4.5 \\ 
netlib & 1200 & 12000 & 2.7 \\ 
fmt\_format & 48 & 510 & 2.8 \\ 
grisu3 & 44 & 470 & 2.9 \\ 
grisu\_exact & 30 & 320 & 2.9 \\ 
schubfach & 30 & 290 & 2.6 \\ 
dragonbox & 24 & 230 & 2.6 \\ 
ryu & 30 & 350 & 3.1 \\ 
teju\_jagua & 30 & 260 & 2.4 \\ 
double\_conversion & 86 & 960 & 3.0 \\ 
swiftDtoa & 37 & 380 & 2.7 \\ 
yy\_double & 25 & 240 & 2.6 \\ 
std::to\_chars & 47 & 640 & 3.7 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 140 & 2200 & 4.2 \\ 
fmt\_format & 40 & 390 & 2.7 \\ 
grisu\_exact & 29 & 270 & 2.5 \\ 
schubfach & 23 & 220 & 2.6 \\ 
dragonbox & 19 & 170 & 2.5 \\ 
ryu & 27 & 290 & 2.8 \\ 
teju\_jagua & 28 & 240 & 2.3 \\ 
double\_conversion & 72 & 800 & 3.0 \\ 
swiftDtoa & 32 & 310 & 2.6 \\ 
std::to\_chars & 41 & 460 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 280 & 4600 & 4.5 \\ 
netlib & 1200 & 12000 & 2.6 \\ 
fmt\_format & 88 & 1100 & 3.5 \\ 
grisu3 & 52 & 680 & 3.5 \\ 
grisu\_exact & 44 & 570 & 3.5 \\ 
schubfach & 46 & 550 & 3.2 \\ 
dragonbox & 34 & 450 & 3.6 \\ 
ryu & 43 & 630 & 3.9 \\ 
teju\_jagua & 44 & 520 & 3.2 \\ 
double\_conversion & 94 & 1100 & 3.0 \\ 
swiftDtoa & 55 & 660 & 3.2 \\ 
yy\_double & 39 & 490 & 3.4 \\ 
std::to\_chars & 57 & 860 & 4.1 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 150 & 2400 & 4.4 \\ 
fmt\_format & 69 & 890 & 3.5 \\ 
grisu\_exact & 40 & 480 & 3.3 \\ 
schubfach & 37 & 460 & 3.3 \\ 
dragonbox & 31 & 380 & 3.3 \\ 
ryu & 38 & 520 & 3.6 \\ 
teju\_jagua & 37 & 450 & 3.3 \\ 
double\_conversion & 80 & 910 & 3.1 \\ 
swiftDtoa & 40 & 490 & 3.3 \\ 
std::to\_chars & 51 & 680 & 3.6 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 2300 & 4.6 \\ 
netlib & 450 & 3900 & 2.4 \\ 
fmt\_format & 48 & 610 & 3.4 \\ 
grisu3 & 23 & 310 & 3.6 \\ 
grisu\_exact & 29 & 390 & 3.6 \\ 
schubfach & 20 & 270 & 3.5 \\ 
dragonbox & 18 & 270 & 3.9 \\ 
ryu & 24 & 350 & 3.8 \\ 
teju\_jagua & 21 & 260 & 3.3 \\ 
double\_conversion & 54 & 630 & 3.2 \\ 
swiftDtoa & 43 & 530 & 3.3 \\ 
yy\_double & 23 & 230 & 2.7 \\ 
std::to\_chars & 37 & 520 & 3.8 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 100 & 1700 & 4.4 \\ 
fmt\_format & 44 & 530 & 3.3 \\ 
grisu\_exact & 27 & 330 & 3.2 \\ 
schubfach & 19 & 230 & 3.3 \\ 
dragonbox & 17 & 210 & 3.4 \\ 
ryu & 29 & 400 & 3.7 \\ 
teju\_jagua & 20 & 240 & 3.2 \\ 
double\_conversion & 57 & 640 & 3.0 \\ 
swiftDtoa & 27 & 310 & 3.1 \\ 
std::to\_chars & 41 & 560 & 3.7 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 290 & 4900 & 4.5 \\ 
netlib & 1300 & 12000 & 2.6 \\ 
fmt\_format & 54 & 590 & 3.0 \\ 
grisu3 & 44 & 520 & 3.2 \\ 
grisu\_exact & 33 & 380 & 3.1 \\ 
schubfach & 34 & 340 & 2.7 \\ 
dragonbox & 24 & 250 & 2.8 \\ 
ryu & 32 & 410 & 3.5 \\ 
teju\_jagua & 32 & 320 & 2.7 \\ 
double\_conversion & 80 & 830 & 2.8 \\ 
swiftDtoa & 46 & 460 & 2.7 \\ 
yy\_double & 30 & 290 & 2.6 \\ 
std::to\_chars & 48 & 640 & 3.6 \\ 
\bottomrule
\end{tabular}


==> results/c6a.metal/AMD_EPYC_7R13_48-Core_Processor_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 160 & 2400 & 4.1 \\ 
fmt\_format & 43 & 460 & 2.9 \\ 
grisu\_exact & 30 & 290 & 2.6 \\ 
schubfach & 24 & 250 & 2.8 \\ 
dragonbox & 19 & 180 & 2.5 \\ 
ryu & 28 & 320 & 3.0 \\ 
teju\_jagua & 27 & 240 & 2.4 \\ 
double\_conversion & 64 & 690 & 2.9 \\ 
swiftDtoa & 31 & 290 & 2.5 \\ 
std::to\_chars & 41 & 460 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 430 & 3300 & 3.1 \\ 
netlib & 2700 & 12000 & 1.7 \\ 
fmt\_format & 140 & 820 & 2.4 \\ 
grisu3 & 100 & 650 & 2.6 \\ 
grisu\_exact & 83 & 550 & 2.7 \\ 
schubfach & 85 & 520 & 2.5 \\ 
dragonbox & 66 & 450 & 2.8 \\ 
ryu & 85 & 540 & 2.6 \\ 
teju\_jagua & 81 & 490 & 2.4 \\ 
double\_conversion & 160 & 1100 & 2.8 \\ 
swiftDtoa & 89 & 560 & 2.6 \\ 
yy\_double & 76 & 430 & 2.3 \\ 
std::to\_chars & 120 & 810 & 2.6 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 230 & 1800 & 3.1 \\ 
fmt\_format & 95 & 720 & 3.1 \\ 
grisu\_exact & 63 & 460 & 3.0 \\ 
schubfach & 64 & 460 & 2.9 \\ 
dragonbox & 55 & 400 & 2.9 \\ 
ryu & 60 & 470 & 3.1 \\ 
teju\_jagua & 64 & 450 & 2.8 \\ 
double\_conversion & 140 & 960 & 2.7 \\ 
swiftDtoa & 67 & 500 & 3.0 \\ 
std::to\_chars & 83 & 640 & 3.1 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 200 & 1600 & 3.1 \\ 
netlib & 940 & 4000 & 1.7 \\ 
fmt\_format & 85 & 530 & 2.5 \\ 
grisu3 & 40 & 290 & 2.9 \\ 
grisu\_exact & 58 & 340 & 2.4 \\ 
schubfach & 33 & 240 & 2.9 \\ 
dragonbox & 40 & 250 & 2.6 \\ 
ryu & 50 & 290 & 2.3 \\ 
teju\_jagua & 36 & 230 & 2.6 \\ 
double\_conversion & 90 & 650 & 2.9 \\ 
swiftDtoa & 65 & 400 & 2.5 \\ 
yy\_double & 30 & 180 & 2.4 \\ 
std::to\_chars & 69 & 480 & 2.8 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 160 & 1200 & 3.1 \\ 
fmt\_format & 59 & 450 & 3.1 \\ 
grisu\_exact & 37 & 270 & 3.0 \\ 
schubfach & 30 & 210 & 2.9 \\ 
dragonbox & 30 & 210 & 2.8 \\ 
ryu & 42 & 330 & 3.1 \\ 
teju\_jagua & 33 & 220 & 2.7 \\ 
double\_conversion & 93 & 650 & 2.8 \\ 
swiftDtoa & 43 & 300 & 2.8 \\ 
std::to\_chars & 65 & 500 & 3.1 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 440 & 3400 & 3.1 \\ 
netlib & 2900 & 13000 & 1.7 \\ 
fmt\_format & 89 & 490 & 2.2 \\ 
grisu3 & 79 & 470 & 2.4 \\ 
grisu\_exact & 57 & 330 & 2.3 \\ 
schubfach & 57 & 290 & 2.0 \\ 
dragonbox & 42 & 230 & 2.2 \\ 
ryu & 57 & 310 & 2.2 \\ 
teju\_jagua & 54 & 260 & 1.9 \\ 
double\_conversion & 120 & 870 & 2.8 \\ 
swiftDtoa & 66 & 360 & 2.2 \\ 
yy\_double & 40 & 200 & 2.0 \\ 
std::to\_chars & 87 & 570 & 2.6 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 230 & 1700 & 3.0 \\ 
fmt\_format & 55 & 390 & 2.8 \\ 
grisu\_exact & 42 & 240 & 2.3 \\ 
schubfach & 41 & 220 & 2.2 \\ 
dragonbox & 31 & 170 & 2.2 \\ 
ryu & 39 & 240 & 2.5 \\ 
teju\_jagua & 46 & 220 & 2.0 \\ 
double\_conversion & 110 & 710 & 2.7 \\ 
swiftDtoa & 50 & 300 & 2.4 \\ 
std::to\_chars & 57 & 410 & 2.9 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 460 & 3600 & 3.1 \\ 
netlib & 2700 & 12000 & 1.8 \\ 
fmt\_format & 170 & 1200 & 2.9 \\ 
grisu3 & 99 & 700 & 2.8 \\ 
grisu\_exact & 93 & 610 & 2.6 \\ 
schubfach & 85 & 540 & 2.6 \\ 
dragonbox & 67 & 470 & 2.8 \\ 
ryu & 87 & 600 & 2.8 \\ 
teju\_jagua & 85 & 530 & 2.5 \\ 
double\_conversion & 160 & 1000 & 2.7 \\ 
swiftDtoa & 91 & 570 & 2.5 \\ 
yy\_double & 74 & 480 & 2.6 \\ 
std::to\_chars & 120 & 810 & 2.7 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 260 & 1900 & 3.0 \\ 
fmt\_format & 120 & 870 & 2.9 \\ 
grisu\_exact & 74 & 510 & 2.8 \\ 
schubfach & 68 & 470 & 2.8 \\ 
dragonbox & 57 & 410 & 2.9 \\ 
ryu & 70 & 500 & 2.9 \\ 
teju\_jagua & 68 & 460 & 2.8 \\ 
double\_conversion & 140 & 900 & 2.6 \\ 
swiftDtoa & 73 & 500 & 2.7 \\ 
std::to\_chars & 87 & 650 & 3.0 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 220 & 1700 & 3.2 \\ 
netlib & 950 & 4000 & 1.7 \\ 
fmt\_format & 88 & 610 & 2.8 \\ 
grisu3 & 40 & 310 & 3.1 \\ 
grisu\_exact & 67 & 410 & 2.4 \\ 
schubfach & 35 & 250 & 2.9 \\ 
dragonbox & 39 & 260 & 2.7 \\ 
ryu & 49 & 330 & 2.7 \\ 
teju\_jagua & 38 & 250 & 2.6 \\ 
double\_conversion & 88 & 610 & 2.8 \\ 
swiftDtoa & 66 & 410 & 2.5 \\ 
yy\_double & 33 & 210 & 2.6 \\ 
std::to\_chars & 71 & 490 & 2.8 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 1300 & 3.2 \\ 
fmt\_format & 72 & 530 & 3.0 \\ 
grisu\_exact & 43 & 320 & 3.0 \\ 
schubfach & 31 & 220 & 3.0 \\ 
dragonbox & 30 & 210 & 2.8 \\ 
ryu & 48 & 350 & 3.0 \\ 
teju\_jagua & 32 & 220 & 2.8 \\ 
double\_conversion & 91 & 610 & 2.7 \\ 
swiftDtoa & 45 & 290 & 2.6 \\ 
std::to\_chars & 66 & 500 & 3.1 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 460 & 3700 & 3.2 \\ 
netlib & 2900 & 13000 & 1.7 \\ 
fmt\_format & 94 & 590 & 2.5 \\ 
grisu3 & 78 & 500 & 2.6 \\ 
grisu\_exact & 66 & 380 & 2.3 \\ 
schubfach & 56 & 300 & 2.1 \\ 
dragonbox & 43 & 230 & 2.2 \\ 
ryu & 57 & 360 & 2.5 \\ 
teju\_jagua & 57 & 290 & 2.1 \\ 
double\_conversion & 120 & 790 & 2.7 \\ 
swiftDtoa & 66 & 360 & 2.2 \\ 
yy\_double & 45 & 250 & 2.2 \\ 
std::to\_chars & 87 & 570 & 2.6 \\ 
\bottomrule
\end{tabular}


==> results/c6g.medium/Neoverse-N1_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 240 & 1800 & 3.1 \\ 
fmt\_format & 70 & 460 & 2.6 \\ 
grisu\_exact & 46 & 280 & 2.4 \\ 
schubfach & 42 & 230 & 2.2 \\ 
dragonbox & 31 & 170 & 2.2 \\ 
ryu & 44 & 270 & 2.5 \\ 
teju\_jagua & 43 & 230 & 2.1 \\ 
double\_conversion & 100 & 650 & 2.6 \\ 
swiftDtoa & 50 & 290 & 2.3 \\ 
std::to\_chars & 58 & 410 & 2.8 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_clang++_all_none.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8375C results (clang++, 64-bit floats)}%
  \label{tab:intelrxeonrplatinum8375ccpu290ghzresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 130 & 2100 & 4.5  & 280 & 4400 & 4.5  & 300 & 4600 & 4.4  \\
    fmt\_format & 44 & 530 & 3.4  & 66 & 830 & 3.6  & 51 & 500 & 2.8  \\
    grisu3 & 22 & 290 & 3.8  & 57 & 630 & 3.2  & 48 & 470 & 2.8  \\
    grisu\_exact & 28 & 340 & 3.5  & 44 & 510 & 3.3  & 31 & 320 & 2.9  \\
    schubfach & 17 & 240 & 4.0  & 43 & 490 & 3.3  & 31 & 290 & 2.7  \\
    dragonbox & 20 & 250 & 3.6  & 34 & 420 & 3.5  & 25 & 220 & 2.6  \\
    ryu & 24 & 310 & 3.6  & 42 & 540 & 3.7  & 31 & 330 & 3.1  \\
    double\_conversion & 61 & 720 & 3.4  & 110 & 1200 & 3.2  & 85 & 960 & 3.2  \\
    swiftDtoa & 34 & 420 & 3.5  & 44 & 540 & 3.5  & 37 & 360 & 2.8  \\
    std::to\_chars & 37 & 510 & 4.0  & 59 & 850 & 4.2  & 50 & 640 & 3.6  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_clang++_all_s.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8375C results (clang++, 32-bit floats)}%
  \label{tab:intelrxeonrplatinum8375ccpu290ghzresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 100 & 1600 & 4.4  & 150 & 2300 & 4.4  & 160 & 2200 & 4.0  \\
    fmt\_format & 40 & 460 & 3.3  & 59 & 730 & 3.6  & 42 & 390 & 2.7  \\
    grisu\_exact & 24 & 300 & 3.5  & 40 & 460 & 3.3  & 32 & 270 & 2.4  \\
    schubfach & 17 & 220 & 3.7  & 35 & 430 & 3.5  & 25 & 230 & 2.5  \\
    dragonbox & 16 & 200 & 3.6  & 30 & 370 & 3.5  & 20 & 170 & 2.5  \\
    ryu & 30 & 380 & 3.6  & 38 & 480 & 3.6  & 31 & 290 & 2.7  \\
    double\_conversion & 62 & 720 & 3.3  & 92 & 1000 & 3.2  & 73 & 800 & 3.1  \\
    swiftDtoa & 24 & 310 & 3.7  & 37 & 490 & 3.8  & 35 & 310 & 2.6  \\
    std::to\_chars & 42 & 550 & 3.8  & 52 & 670 & 3.7  & 42 & 460 & 3.1  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 280 & 4400 & 4.5 \\ 
netlib & 1300 & 12000 & 2.4 \\ 
fmt\_format & 66 & 830 & 3.6 \\ 
grisu3 & 57 & 630 & 3.2 \\ 
grisu\_exact & 44 & 510 & 3.3 \\ 
schubfach & 43 & 490 & 3.3 \\ 
dragonbox & 34 & 420 & 3.5 \\ 
ryu & 42 & 540 & 3.7 \\ 
teju\_jagua & 44 & 470 & 3.0 \\ 
double\_conversion & 110 & 1200 & 3.2 \\ 
swiftDtoa & 44 & 540 & 3.5 \\ 
yy\_double & 36 & 430 & 3.4 \\ 
std::to\_chars & 59 & 850 & 4.2 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 150 & 2300 & 4.4 \\ 
fmt\_format & 59 & 730 & 3.6 \\ 
grisu\_exact & 40 & 460 & 3.3 \\ 
schubfach & 35 & 430 & 3.5 \\ 
dragonbox & 30 & 370 & 3.5 \\ 
ryu & 38 & 480 & 3.6 \\ 
teju\_jagua & 40 & 440 & 3.1 \\ 
double\_conversion & 92 & 1000 & 3.2 \\ 
swiftDtoa & 37 & 490 & 3.8 \\ 
std::to\_chars & 52 & 670 & 3.7 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 2100 & 4.5 \\ 
netlib & 480 & 3900 & 2.4 \\ 
fmt\_format & 44 & 530 & 3.4 \\ 
grisu3 & 22 & 290 & 3.8 \\ 
grisu\_exact & 28 & 340 & 3.5 \\ 
schubfach & 17 & 240 & 4.0 \\ 
dragonbox & 20 & 250 & 3.6 \\ 
ryu & 24 & 310 & 3.6 \\ 
teju\_jagua & 20 & 230 & 3.4 \\ 
double\_conversion & 61 & 720 & 3.4 \\ 
swiftDtoa & 34 & 420 & 3.5 \\ 
yy\_double & 15 & 190 & 3.6 \\ 
std::to\_chars & 37 & 510 & 4.0 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 100 & 1600 & 4.4 \\ 
fmt\_format & 40 & 460 & 3.3 \\ 
grisu\_exact & 24 & 300 & 3.5 \\ 
schubfach & 17 & 220 & 3.7 \\ 
dragonbox & 16 & 200 & 3.6 \\ 
ryu & 30 & 380 & 3.6 \\ 
teju\_jagua & 20 & 230 & 3.4 \\ 
double\_conversion & 62 & 720 & 3.3 \\ 
swiftDtoa & 24 & 310 & 3.7 \\ 
std::to\_chars & 42 & 550 & 3.8 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 300 & 4600 & 4.4 \\ 
netlib & 1400 & 12000 & 2.5 \\ 
fmt\_format & 51 & 500 & 2.8 \\ 
grisu3 & 48 & 470 & 2.8 \\ 
grisu\_exact & 31 & 320 & 2.9 \\ 
schubfach & 31 & 290 & 2.7 \\ 
dragonbox & 25 & 220 & 2.6 \\ 
ryu & 31 & 330 & 3.1 \\ 
teju\_jagua & 31 & 270 & 2.4 \\ 
double\_conversion & 85 & 960 & 3.2 \\ 
swiftDtoa & 37 & 360 & 2.8 \\ 
yy\_double & 23 & 230 & 2.9 \\ 
std::to\_chars & 50 & 640 & 3.6 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 160 & 2200 & 4.0 \\ 
fmt\_format & 42 & 390 & 2.7 \\ 
grisu\_exact & 32 & 270 & 2.4 \\ 
schubfach & 25 & 230 & 2.5 \\ 
dragonbox & 20 & 170 & 2.5 \\ 
ryu & 31 & 290 & 2.7 \\ 
teju\_jagua & 31 & 240 & 2.2 \\ 
double\_conversion & 73 & 800 & 3.1 \\ 
swiftDtoa & 35 & 310 & 2.6 \\ 
std::to\_chars & 42 & 460 & 3.1 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_g++_all_none.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8375C results (g++, 64-bit floats)}%
  \label{tab:intelrxeonrplatinum8375ccpu290ghzresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 140 & 2200 & 4.5  & 290 & 4600 & 4.5  & 320 & 4900 & 4.4  \\
    fmt\_format & 51 & 610 & 3.4  & 90 & 1200 & 3.7  & 59 & 590 & 2.9  \\
    grisu3 & 24 & 310 & 3.7  & 56 & 680 & 3.4  & 49 & 520 & 3.0  \\
    grisu\_exact & 31 & 390 & 3.6  & 46 & 570 & 3.6  & 36 & 380 & 3.0  \\
    schubfach & 19 & 270 & 4.1  & 45 & 550 & 3.5  & 33 & 340 & 3.0  \\
    dragonbox & 18 & 270 & 4.2  & 34 & 450 & 3.8  & 25 & 250 & 2.8  \\
    ryu & 26 & 350 & 3.8  & 45 & 620 & 3.9  & 33 & 400 & 3.4  \\
    double\_conversion & 54 & 630 & 3.3  & 94 & 1000 & 3.2  & 77 & 830 & 3.1  \\
    swiftDtoa & 41 & 520 & 3.6  & 53 & 650 & 3.6  & 46 & 460 & 2.9  \\
    std::to\_chars & 37 & 510 & 4.0  & 59 & 860 & 4.2  & 50 & 640 & 3.6  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_g++_all_s.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8375C results (g++, 32-bit floats)}%
  \label{tab:intelrxeonrplatinum8375ccpu290ghzresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 110 & 1700 & 4.3  & 160 & 2400 & 4.3  & 180 & 2300 & 3.8  \\
    fmt\_format & 45 & 530 & 3.3  & 72 & 890 & 3.6  & 47 & 460 & 2.8  \\
    grisu\_exact & 28 & 330 & 3.4  & 41 & 480 & 3.3  & 32 & 290 & 2.6  \\
    schubfach & 18 & 230 & 3.7  & 36 & 450 & 3.6  & 26 & 250 & 2.7  \\
    dragonbox & 16 & 210 & 3.8  & 32 & 380 & 3.5  & 20 & 180 & 2.5  \\
    ryu & 30 & 400 & 3.8  & 38 & 520 & 3.9  & 30 & 320 & 3.0  \\
    double\_conversion & 58 & 640 & 3.2  & 84 & 910 & 3.1  & 68 & 680 & 2.9  \\
    swiftDtoa & 25 & 300 & 3.4  & 38 & 490 & 3.6  & 33 & 290 & 2.5  \\
    std::to\_chars & 43 & 560 & 3.7  & 55 & 680 & 3.5  & 42 & 460 & 3.2  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 290 & 4600 & 4.5 \\ 
netlib & 1400 & 12000 & 2.4 \\ 
fmt\_format & 90 & 1200 & 3.7 \\ 
grisu3 & 56 & 680 & 3.4 \\ 
grisu\_exact & 46 & 570 & 3.6 \\ 
schubfach & 45 & 550 & 3.5 \\ 
dragonbox & 34 & 450 & 3.8 \\ 
ryu & 45 & 620 & 3.9 \\ 
teju\_jagua & 46 & 520 & 3.2 \\ 
double\_conversion & 94 & 1000 & 3.2 \\ 
swiftDtoa & 53 & 650 & 3.6 \\ 
yy\_double & 38 & 490 & 3.6 \\ 
std::to\_chars & 59 & 860 & 4.2 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 160 & 2400 & 4.3 \\ 
fmt\_format & 72 & 890 & 3.6 \\ 
grisu\_exact & 41 & 480 & 3.3 \\ 
schubfach & 36 & 450 & 3.6 \\ 
dragonbox & 32 & 380 & 3.5 \\ 
ryu & 38 & 520 & 3.9 \\ 
teju\_jagua & 38 & 450 & 3.4 \\ 
double\_conversion & 84 & 910 & 3.1 \\ 
swiftDtoa & 38 & 490 & 3.6 \\ 
std::to\_chars & 55 & 680 & 3.5 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 140 & 2200 & 4.5 \\ 
netlib & 470 & 3900 & 2.4 \\ 
fmt\_format & 51 & 610 & 3.4 \\ 
grisu3 & 24 & 310 & 3.7 \\ 
grisu\_exact & 31 & 390 & 3.6 \\ 
schubfach & 19 & 270 & 4.1 \\ 
dragonbox & 18 & 270 & 4.2 \\ 
ryu & 26 & 350 & 3.8 \\ 
teju\_jagua & 20 & 260 & 3.7 \\ 
double\_conversion & 54 & 630 & 3.3 \\ 
swiftDtoa & 41 & 520 & 3.6 \\ 
yy\_double & 19 & 230 & 3.5 \\ 
std::to\_chars & 37 & 510 & 4.0 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 110 & 1700 & 4.3 \\ 
fmt\_format & 45 & 530 & 3.3 \\ 
grisu\_exact & 28 & 330 & 3.4 \\ 
schubfach & 18 & 230 & 3.7 \\ 
dragonbox & 16 & 210 & 3.8 \\ 
ryu & 30 & 400 & 3.8 \\ 
teju\_jagua & 19 & 240 & 3.6 \\ 
double\_conversion & 58 & 640 & 3.2 \\ 
swiftDtoa & 25 & 300 & 3.4 \\ 
std::to\_chars & 43 & 560 & 3.7 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 320 & 4900 & 4.4 \\ 
netlib & 1500 & 12000 & 2.4 \\ 
fmt\_format & 59 & 590 & 2.9 \\ 
grisu3 & 49 & 520 & 3.0 \\ 
grisu\_exact & 36 & 380 & 3.0 \\ 
schubfach & 33 & 340 & 3.0 \\ 
dragonbox & 25 & 250 & 2.8 \\ 
ryu & 33 & 400 & 3.4 \\ 
teju\_jagua & 33 & 320 & 2.7 \\ 
double\_conversion & 77 & 830 & 3.1 \\ 
swiftDtoa & 46 & 460 & 2.9 \\ 
yy\_double & 31 & 280 & 2.6 \\ 
std::to\_chars & 50 & 640 & 3.6 \\ 
\bottomrule
\end{tabular}


==> results/c6i.metal/Intel_R__Xeon_R__Platinum_8375C_CPU__2.90GHz_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 180 & 2300 & 3.8 \\ 
fmt\_format & 47 & 460 & 2.8 \\ 
grisu\_exact & 32 & 290 & 2.6 \\ 
schubfach & 26 & 250 & 2.7 \\ 
dragonbox & 20 & 180 & 2.5 \\ 
ryu & 30 & 320 & 3.0 \\ 
teju\_jagua & 29 & 240 & 2.4 \\ 
double\_conversion & 68 & 680 & 2.9 \\ 
swiftDtoa & 33 & 290 & 2.5 \\ 
std::to\_chars & 42 & 460 & 3.2 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 250 & 4400 & 4.7 \\ 
netlib & 1100 & 12000 & 2.8 \\ 
fmt\_format & 63 & 860 & 3.7 \\ 
grisu3 & 50 & 630 & 3.4 \\ 
grisu\_exact & 39 & 510 & 3.6 \\ 
schubfach & 39 & 490 & 3.5 \\ 
dragonbox & 31 & 420 & 3.6 \\ 
ryu & 39 & 560 & 3.8 \\ 
teju\_jagua & 39 & 470 & 3.3 \\ 
double\_conversion & 91 & 1200 & 3.6 \\ 
swiftDtoa & 43 & 560 & 3.5 \\ 
yy\_double & 32 & 430 & 3.6 \\ 
std::to\_chars & 52 & 850 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 120 & 2300 & 5.0 \\ 
fmt\_format & 54 & 730 & 3.6 \\ 
grisu\_exact & 35 & 460 & 3.6 \\ 
schubfach & 31 & 430 & 3.8 \\ 
dragonbox & 28 & 370 & 3.7 \\ 
ryu & 34 & 480 & 3.8 \\ 
teju\_jagua & 35 & 440 & 3.4 \\ 
double\_conversion & 80 & 1000 & 3.5 \\ 
swiftDtoa & 34 & 490 & 3.9 \\ 
std::to\_chars & 46 & 670 & 4.0 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 120 & 2100 & 4.9 \\ 
netlib & 420 & 3900 & 2.6 \\ 
fmt\_format & 42 & 540 & 3.5 \\ 
grisu3 & 21 & 290 & 3.8 \\ 
grisu\_exact & 24 & 340 & 3.8 \\ 
schubfach & 17 & 240 & 3.9 \\ 
dragonbox & 18 & 250 & 3.8 \\ 
ryu & 22 & 310 & 3.9 \\ 
teju\_jagua & 18 & 240 & 3.5 \\ 
double\_conversion & 54 & 720 & 3.6 \\ 
swiftDtoa & 32 & 440 & 3.7 \\ 
yy\_double & 15 & 190 & 3.4 \\ 
std::to\_chars & 32 & 510 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 87 & 1600 & 4.9 \\ 
fmt\_format & 36 & 460 & 3.5 \\ 
grisu\_exact & 23 & 300 & 3.6 \\ 
schubfach & 16 & 220 & 3.6 \\ 
dragonbox & 15 & 200 & 3.7 \\ 
ryu & 27 & 380 & 3.8 \\ 
teju\_jagua & 18 & 230 & 3.4 \\ 
double\_conversion & 55 & 730 & 3.6 \\ 
swiftDtoa & 23 & 310 & 3.7 \\ 
std::to\_chars & 37 & 550 & 4.1 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 250 & 4600 & 4.9 \\ 
netlib & 1200 & 12000 & 2.8 \\ 
fmt\_format & 47 & 510 & 2.9 \\ 
grisu3 & 44 & 470 & 2.9 \\ 
grisu\_exact & 30 & 320 & 2.9 \\ 
schubfach & 31 & 290 & 2.5 \\ 
dragonbox & 24 & 230 & 2.6 \\ 
ryu & 31 & 350 & 3.1 \\ 
teju\_jagua & 29 & 260 & 2.5 \\ 
double\_conversion & 78 & 970 & 3.4 \\ 
swiftDtoa & 36 & 370 & 2.8 \\ 
yy\_double & 22 & 240 & 2.9 \\ 
std::to\_chars & 45 & 640 & 3.9 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 2200 & 4.6 \\ 
fmt\_format & 38 & 390 & 2.8 \\ 
grisu\_exact & 29 & 270 & 2.5 \\ 
schubfach & 23 & 220 & 2.6 \\ 
dragonbox & 19 & 170 & 2.5 \\ 
ryu & 28 & 290 & 2.8 \\ 
teju\_jagua & 28 & 240 & 2.3 \\ 
double\_conversion & 66 & 800 & 3.3 \\ 
swiftDtoa & 31 & 310 & 2.7 \\ 
std::to\_chars & 38 & 460 & 3.3 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 260 & 4700 & 4.9 \\ 
netlib & 1100 & 12000 & 2.9 \\ 
fmt\_format & 83 & 1200 & 4.0 \\ 
grisu3 & 49 & 680 & 3.8 \\ 
grisu\_exact & 41 & 580 & 3.8 \\ 
schubfach & 43 & 550 & 3.5 \\ 
dragonbox & 32 & 450 & 3.8 \\ 
ryu & 42 & 630 & 4.1 \\ 
teju\_jagua & 41 & 530 & 3.5 \\ 
double\_conversion & 80 & 1100 & 3.6 \\ 
swiftDtoa & 53 & 660 & 3.4 \\ 
yy\_double & 37 & 480 & 3.6 \\ 
std::to\_chars & 53 & 860 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 2400 & 5.0 \\ 
fmt\_format & 62 & 910 & 4.0 \\ 
grisu\_exact & 38 & 490 & 3.5 \\ 
schubfach & 32 & 460 & 3.9 \\ 
dragonbox & 29 & 390 & 3.6 \\ 
ryu & 35 & 520 & 4.0 \\ 
teju\_jagua & 35 & 450 & 3.5 \\ 
double\_conversion & 71 & 920 & 3.5 \\ 
swiftDtoa & 37 & 490 & 3.6 \\ 
std::to\_chars & 47 & 680 & 4.0 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 2300 & 4.9 \\ 
netlib & 400 & 3900 & 2.7 \\ 
fmt\_format & 46 & 610 & 3.6 \\ 
grisu3 & 21 & 310 & 3.9 \\ 
grisu\_exact & 28 & 390 & 3.8 \\ 
schubfach & 19 & 270 & 3.8 \\ 
dragonbox & 17 & 270 & 4.4 \\ 
ryu & 22 & 350 & 4.3 \\ 
teju\_jagua & 20 & 260 & 3.6 \\ 
double\_conversion & 48 & 640 & 3.6 \\ 
swiftDtoa & 41 & 530 & 3.5 \\ 
yy\_double & 20 & 230 & 3.1 \\ 
std::to\_chars & 32 & 510 & 4.3 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 99 & 1700 & 4.6 \\ 
fmt\_format & 39 & 530 & 3.7 \\ 
grisu\_exact & 25 & 330 & 3.6 \\ 
schubfach & 17 & 240 & 3.8 \\ 
dragonbox & 15 & 220 & 3.9 \\ 
ryu & 28 & 400 & 3.9 \\ 
teju\_jagua & 18 & 250 & 3.6 \\ 
double\_conversion & 46 & 640 & 3.8 \\ 
swiftDtoa & 24 & 310 & 3.4 \\ 
std::to\_chars & 37 & 560 & 4.1 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 280 & 4900 & 4.8 \\ 
netlib & 1100 & 12000 & 2.9 \\ 
fmt\_format & 52 & 590 & 3.1 \\ 
grisu3 & 42 & 520 & 3.4 \\ 
grisu\_exact & 33 & 380 & 3.2 \\ 
schubfach & 32 & 340 & 2.8 \\ 
dragonbox & 24 & 250 & 2.8 \\ 
ryu & 32 & 410 & 3.5 \\ 
teju\_jagua & 30 & 320 & 2.8 \\ 
double\_conversion & 70 & 840 & 3.2 \\ 
swiftDtoa & 45 & 460 & 2.8 \\ 
yy\_double & 30 & 280 & 2.5 \\ 
std::to\_chars & 46 & 640 & 3.8 \\ 
\bottomrule
\end{tabular}


==> results/c7a.metal-48xl/AMD_EPYC_9R14_96-Core_Processor_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 150 & 2400 & 4.2 \\ 
fmt\_format & 41 & 460 & 3.0 \\ 
grisu\_exact & 30 & 290 & 2.6 \\ 
schubfach & 24 & 250 & 2.8 \\ 
dragonbox & 19 & 180 & 2.6 \\ 
ryu & 28 & 320 & 3.1 \\ 
teju\_jagua & 27 & 240 & 2.5 \\ 
double\_conversion & 57 & 690 & 3.3 \\ 
swiftDtoa & 31 & 290 & 2.6 \\ 
std::to\_chars & 38 & 460 & 3.3 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 290 & 3300 & 4.4 \\ 
netlib & 2500 & 12000 & 1.8 \\ 
fmt\_format & 85 & 820 & 3.7 \\ 
grisu3 & 67 & 650 & 3.7 \\ 
grisu\_exact & 54 & 550 & 3.9 \\ 
schubfach & 50 & 520 & 4.0 \\ 
dragonbox & 41 & 450 & 4.2 \\ 
ryu & 51 & 540 & 4.1 \\ 
teju\_jagua & 50 & 490 & 3.8 \\ 
double\_conversion & 120 & 1100 & 3.6 \\ 
swiftDtoa & 53 & 560 & 4.1 \\ 
yy\_double & 42 & 430 & 3.9 \\ 
std::to\_chars & 69 & 800 & 4.5 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 160 & 1800 & 4.2 \\ 
fmt\_format & 66 & 720 & 4.3 \\ 
grisu\_exact & 44 & 460 & 4.0 \\ 
schubfach & 41 & 450 & 4.2 \\ 
dragonbox & 37 & 400 & 4.1 \\ 
ryu & 41 & 460 & 4.3 \\ 
teju\_jagua & 44 & 450 & 3.9 \\ 
double\_conversion & 98 & 950 & 3.7 \\ 
swiftDtoa & 42 & 490 & 4.5 \\ 
std::to\_chars & 53 & 640 & 4.6 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 140 & 1600 & 4.4 \\ 
netlib & 920 & 4000 & 1.7 \\ 
fmt\_format & 59 & 530 & 3.5 \\ 
grisu3 & 30 & 290 & 3.8 \\ 
grisu\_exact & 35 & 340 & 3.7 \\ 
schubfach & 22 & 230 & 4.1 \\ 
dragonbox & 26 & 250 & 3.7 \\ 
ryu & 29 & 290 & 3.7 \\ 
teju\_jagua & 23 & 230 & 3.8 \\ 
double\_conversion & 68 & 640 & 3.6 \\ 
swiftDtoa & 43 & 400 & 3.6 \\ 
yy\_double & 19 & 170 & 3.5 \\ 
std::to\_chars & 42 & 480 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 110 & 1200 & 4.3 \\ 
fmt\_format & 46 & 450 & 3.8 \\ 
grisu\_exact & 28 & 270 & 3.7 \\ 
schubfach & 20 & 210 & 4.0 \\ 
dragonbox & 21 & 200 & 3.7 \\ 
ryu & 33 & 320 & 3.8 \\ 
teju\_jagua & 23 & 220 & 3.6 \\ 
double\_conversion & 69 & 650 & 3.6 \\ 
swiftDtoa & 31 & 290 & 3.6 \\ 
std::to\_chars & 44 & 500 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 310 & 3400 & 4.3 \\ 
netlib & 2800 & 13000 & 1.8 \\ 
fmt\_format & 56 & 490 & 3.4 \\ 
grisu3 & 56 & 470 & 3.2 \\ 
grisu\_exact & 41 & 330 & 3.1 \\ 
schubfach & 36 & 290 & 3.1 \\ 
dragonbox & 27 & 230 & 3.2 \\ 
ryu & 35 & 310 & 3.4 \\ 
teju\_jagua & 36 & 260 & 2.8 \\ 
double\_conversion & 93 & 870 & 3.6 \\ 
swiftDtoa & 43 & 360 & 3.2 \\ 
yy\_double & 25 & 200 & 3.1 \\ 
std::to\_chars & 53 & 570 & 4.1 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 160 & 1700 & 4.0 \\ 
fmt\_format & 40 & 390 & 3.8 \\ 
grisu\_exact & 33 & 240 & 2.8 \\ 
schubfach & 29 & 220 & 3.0 \\ 
dragonbox & 23 & 170 & 3.0 \\ 
ryu & 29 & 240 & 3.2 \\ 
teju\_jagua & 33 & 220 & 2.6 \\ 
double\_conversion & 79 & 710 & 3.5 \\ 
swiftDtoa & 35 & 300 & 3.2 \\ 
std::to\_chars & 42 & 410 & 3.8 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 300 & 3500 & 4.5 \\ 
netlib & 2600 & 12000 & 1.7 \\ 
fmt\_format & 110 & 1200 & 4.2 \\ 
grisu3 & 65 & 690 & 4.1 \\ 
grisu\_exact & 56 & 610 & 4.2 \\ 
schubfach & 49 & 540 & 4.3 \\ 
dragonbox & 41 & 460 & 4.3 \\ 
ryu & 51 & 600 & 4.5 \\ 
teju\_jagua & 53 & 530 & 3.9 \\ 
double\_conversion & 100 & 1000 & 3.8 \\ 
swiftDtoa & 52 & 560 & 4.2 \\ 
yy\_double & 43 & 480 & 4.3 \\ 
std::to\_chars & 72 & 810 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 1900 & 4.3 \\ 
fmt\_format & 89 & 870 & 3.8 \\ 
grisu\_exact & 46 & 500 & 4.2 \\ 
schubfach & 40 & 470 & 4.6 \\ 
dragonbox & 36 & 410 & 4.4 \\ 
ryu & 43 & 500 & 4.5 \\ 
teju\_jagua & 44 & 460 & 4.0 \\ 
double\_conversion & 88 & 890 & 3.9 \\ 
swiftDtoa & 44 & 490 & 4.3 \\ 
std::to\_chars & 54 & 640 & 4.6 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 150 & 1700 & 4.5 \\ 
netlib & 900 & 4000 & 1.7 \\ 
fmt\_format & 59 & 610 & 4.0 \\ 
grisu3 & 27 & 310 & 4.4 \\ 
grisu\_exact & 38 & 400 & 4.1 \\ 
schubfach & 20 & 250 & 4.7 \\ 
dragonbox & 24 & 250 & 4.1 \\ 
ryu & 30 & 320 & 4.2 \\ 
teju\_jagua & 23 & 250 & 4.0 \\ 
double\_conversion & 59 & 600 & 3.9 \\ 
swiftDtoa & 43 & 410 & 3.7 \\ 
yy\_double & 20 & 210 & 3.9 \\ 
std::to\_chars & 42 & 480 & 4.5 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 120 & 1300 & 4.4 \\ 
fmt\_format & 54 & 520 & 3.7 \\ 
grisu\_exact & 29 & 310 & 4.2 \\ 
schubfach & 19 & 220 & 4.5 \\ 
dragonbox & 20 & 200 & 3.9 \\ 
ryu & 33 & 350 & 4.2 \\ 
teju\_jagua & 23 & 220 & 3.7 \\ 
double\_conversion & 60 & 610 & 3.9 \\ 
swiftDtoa & 29 & 290 & 3.8 \\ 
std::to\_chars & 44 & 500 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 320 & 3600 & 4.4 \\ 
netlib & 2800 & 13000 & 1.7 \\ 
fmt\_format & 63 & 590 & 3.6 \\ 
grisu3 & 55 & 500 & 3.5 \\ 
grisu\_exact & 42 & 380 & 3.4 \\ 
schubfach & 34 & 300 & 3.3 \\ 
dragonbox & 28 & 230 & 3.2 \\ 
ryu & 36 & 360 & 3.8 \\ 
teju\_jagua & 38 & 290 & 3.0 \\ 
double\_conversion & 81 & 780 & 3.7 \\ 
swiftDtoa & 43 & 360 & 3.2 \\ 
yy\_double & 31 & 240 & 3.1 \\ 
std::to\_chars & 53 & 570 & 4.1 \\ 
\bottomrule
\end{tabular}


==> results/c7g.medium/Neoverse-V1_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 170 & 1800 & 4.0 \\ 
fmt\_format & 51 & 460 & 3.5 \\ 
grisu\_exact & 34 & 280 & 3.2 \\ 
schubfach & 26 & 230 & 3.5 \\ 
dragonbox & 22 & 170 & 3.0 \\ 
ryu & 30 & 270 & 3.4 \\ 
teju\_jagua & 33 & 230 & 2.7 \\ 
double\_conversion & 69 & 650 & 3.6 \\ 
swiftDtoa & 36 & 290 & 3.1 \\ 
std::to\_chars & 42 & 410 & 3.8 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_clang++_all_none.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8488C results (clang++, 64-bit floats)}%
  \label{tab:intelrxeonrplatinum8488cresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 110 & 2100 & 5.1  & 220 & 4400 & 5.3  & 240 & 4600 & 5.0  \\
    fmt\_format & 33 & 530 & 4.2  & 48 & 830 & 4.6  & 40 & 500 & 3.3  \\
    grisu3 & 18 & 290 & 4.2  & 46 & 630 & 3.6  & 42 & 470 & 2.9  \\
    grisu\_exact & 20 & 340 & 4.5  & 32 & 510 & 4.2  & 26 & 320 & 3.3  \\
    schubfach & 14 & 240 & 4.6  & 34 & 500 & 3.8  & 27 & 290 & 2.8  \\
    dragonbox & 16 & 250 & 4.0  & 26 & 420 & 4.3  & 20 & 220 & 2.9  \\
    ryu & 18 & 310 & 4.5  & 31 & 550 & 4.7  & 24 & 330 & 3.6  \\
    double\_conversion & 45 & 720 & 4.2  & 77 & 1200 & 4.1  & 67 & 960 & 3.8  \\
    swiftDtoa & 27 & 420 & 4.1  & 35 & 540 & 4.1  & 31 & 360 & 3.0  \\
    std::to\_chars & 27 & 510 & 5.0  & 44 & 850 & 5.1  & 38 & 640 & 4.4  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_clang++_all_s.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8488C results (clang++, 32-bit floats)}%
  \label{tab:intelrxeonrplatinum8488cresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 83 & 1600 & 5.0  & 120 & 2300 & 5.2  & 130 & 2200 & 4.5  \\
    fmt\_format & 27 & 460 & 4.5  & 42 & 730 & 4.6  & 31 & 390 & 3.4  \\
    grisu\_exact & 19 & 300 & 4.2  & 31 & 460 & 3.9  & 28 & 270 & 2.6  \\
    schubfach & 15 & 220 & 4.0  & 27 & 430 & 4.2  & 22 & 230 & 2.7  \\
    dragonbox & 13 & 210 & 4.2  & 25 & 370 & 3.9  & 17 & 170 & 2.7  \\
    ryu & 22 & 380 & 4.5  & 29 & 480 & 4.3  & 24 & 290 & 3.2  \\
    double\_conversion & 47 & 730 & 4.1  & 68 & 1000 & 4.0  & 56 & 800 & 3.7  \\
    swiftDtoa & 19 & 310 & 4.3  & 29 & 490 & 4.5  & 29 & 310 & 2.9  \\
    std::to\_chars & 31 & 550 & 4.6  & 39 & 670 & 4.5  & 34 & 460 & 3.6  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 220 & 4400 & 5.3 \\ 
netlib & 760 & 12000 & 4.0 \\ 
fmt\_format & 48 & 830 & 4.6 \\ 
grisu3 & 46 & 630 & 3.6 \\ 
grisu\_exact & 32 & 510 & 4.2 \\ 
schubfach & 34 & 500 & 3.8 \\ 
dragonbox & 26 & 420 & 4.3 \\ 
ryu & 31 & 550 & 4.7 \\ 
teju\_jagua & 34 & 470 & 3.6 \\ 
double\_conversion & 77 & 1200 & 4.1 \\ 
swiftDtoa & 35 & 540 & 4.1 \\ 
yy\_double & 24 & 430 & 4.6 \\ 
std::to\_chars & 44 & 850 & 5.1 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 120 & 2300 & 5.2 \\ 
fmt\_format & 42 & 730 & 4.6 \\ 
grisu\_exact & 31 & 460 & 3.9 \\ 
schubfach & 27 & 430 & 4.2 \\ 
dragonbox & 25 & 370 & 3.9 \\ 
ryu & 29 & 480 & 4.3 \\ 
teju\_jagua & 31 & 440 & 3.7 \\ 
double\_conversion & 68 & 1000 & 4.0 \\ 
swiftDtoa & 29 & 490 & 4.5 \\ 
std::to\_chars & 39 & 670 & 4.5 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 110 & 2100 & 5.1 \\ 
netlib & 300 & 3900 & 3.4 \\ 
fmt\_format & 33 & 530 & 4.2 \\ 
grisu3 & 18 & 290 & 4.2 \\ 
grisu\_exact & 20 & 340 & 4.5 \\ 
schubfach & 14 & 240 & 4.6 \\ 
dragonbox & 16 & 250 & 4.0 \\ 
ryu & 18 & 310 & 4.5 \\ 
teju\_jagua & 16 & 240 & 4.0 \\ 
double\_conversion & 45 & 720 & 4.2 \\ 
swiftDtoa & 27 & 420 & 4.1 \\ 
yy\_double & 11 & 190 & 4.6 \\ 
std::to\_chars & 27 & 510 & 5.0 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 83 & 1600 & 5.0 \\ 
fmt\_format & 27 & 460 & 4.5 \\ 
grisu\_exact & 19 & 300 & 4.2 \\ 
schubfach & 15 & 220 & 4.0 \\ 
dragonbox & 13 & 210 & 4.2 \\ 
ryu & 22 & 380 & 4.5 \\ 
teju\_jagua & 16 & 230 & 3.8 \\ 
double\_conversion & 47 & 730 & 4.1 \\ 
swiftDtoa & 19 & 310 & 4.3 \\ 
std::to\_chars & 31 & 550 & 4.6 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 240 & 4600 & 5.0 \\ 
netlib & 790 & 12000 & 4.1 \\ 
fmt\_format & 40 & 500 & 3.3 \\ 
grisu3 & 42 & 470 & 2.9 \\ 
grisu\_exact & 26 & 320 & 3.3 \\ 
schubfach & 27 & 290 & 2.8 \\ 
dragonbox & 20 & 220 & 2.9 \\ 
ryu & 24 & 330 & 3.6 \\ 
teju\_jagua & 26 & 260 & 2.7 \\ 
double\_conversion & 67 & 960 & 3.8 \\ 
swiftDtoa & 31 & 360 & 3.0 \\ 
yy\_double & 16 & 230 & 3.8 \\ 
std::to\_chars & 38 & 640 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 2200 & 4.5 \\ 
fmt\_format & 31 & 390 & 3.4 \\ 
grisu\_exact & 28 & 270 & 2.6 \\ 
schubfach & 22 & 230 & 2.7 \\ 
dragonbox & 17 & 170 & 2.7 \\ 
ryu & 24 & 290 & 3.2 \\ 
teju\_jagua & 27 & 240 & 2.4 \\ 
double\_conversion & 56 & 800 & 3.7 \\ 
swiftDtoa & 29 & 310 & 2.9 \\ 
std::to\_chars & 34 & 460 & 3.6 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_g++_all_none.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8488C results (g++, 64-bit floats)}%
  \label{tab:intelrxeonrplatinum8488cresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 110 & 2300 & 5.2  & 230 & 4600 & 5.3  & 260 & 4900 & 5.0  \\
    fmt\_format & 35 & 610 & 4.6  & 66 & 1200 & 4.7  & 43 & 590 & 3.6  \\
    grisu3 & 19 & 310 & 4.3  & 46 & 680 & 3.8  & 43 & 520 & 3.2  \\
    grisu\_exact & 23 & 390 & 4.5  & 34 & 570 & 4.5  & 28 & 380 & 3.6  \\
    schubfach & 15 & 270 & 4.7  & 36 & 550 & 4.0  & 28 & 340 & 3.2  \\
    dragonbox & 14 & 270 & 5.1  & 27 & 450 & 4.5  & 21 & 250 & 3.2  \\
    ryu & 19 & 350 & 4.9  & 33 & 620 & 5.0  & 26 & 400 & 4.1  \\
    double\_conversion & 42 & 630 & 4.0  & 75 & 1100 & 3.7  & 63 & 830 & 3.5  \\
    swiftDtoa & 31 & 530 & 4.4  & 41 & 660 & 4.3  & 36 & 470 & 3.4  \\
    std::to\_chars & 27 & 520 & 5.0  & 46 & 860 & 5.0  & 38 & 640 & 4.4  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_g++_all_s.tex <==
\begin{table}
  \centering
  \caption{Intel Xeon 8488C results (g++, 32-bit floats)}%
  \label{tab:intelrxeonrplatinum8488cresults}
  \begin{tabular}{lccccccccc}
    \toprule
    \multirow{1}{*}{Name}   & \multicolumn{3}{c|}{mesh}  & \multicolumn{3}{c|}{canada} & \multicolumn{3}{c}{unit} \\
                            & {ns/f} & {ins/f} & {ins/c} & {ns/f} & {ins/f} & {ins/c}  & {ns/f} & {ins/f} & {ins/c} \\ \midrule
    dragon4 & 88 & 1700 & 5.0  & 130 & 2400 & 5.0  & 140 & 2300 & 4.3  \\
    fmt\_format & 30 & 530 & 4.6  & 54 & 900 & 4.4  & 34 & 460 & 3.5  \\
    grisu\_exact & 22 & 330 & 3.9  & 33 & 490 & 3.8  & 27 & 290 & 2.8  \\
    schubfach & 15 & 240 & 4.2  & 28 & 460 & 4.3  & 23 & 250 & 2.9  \\
    dragonbox & 13 & 220 & 4.3  & 26 & 390 & 3.8  & 17 & 180 & 2.7  \\
    ryu & 22 & 400 & 4.7  & 31 & 520 & 4.4  & 24 & 320 & 3.4  \\
    double\_conversion & 44 & 640 & 3.9  & 65 & 910 & 3.7  & 53 & 680 & 3.4  \\
    swiftDtoa & 20 & 310 & 4.0  & 31 & 490 & 4.1  & 28 & 290 & 2.7  \\
    std::to\_chars & 32 & 560 & 4.6  & 40 & 680 & 4.5  & 34 & 460 & 3.6  \\
    \bottomrule
  \end{tabular}\restartrowcolors
\end{table}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 230 & 4600 & 5.3 \\ 
netlib & 740 & 12000 & 4.1 \\ 
fmt\_format & 66 & 1200 & 4.7 \\ 
grisu3 & 46 & 680 & 3.8 \\ 
grisu\_exact & 34 & 570 & 4.5 \\ 
schubfach & 36 & 550 & 4.0 \\ 
dragonbox & 27 & 450 & 4.5 \\ 
ryu & 33 & 620 & 5.0 \\ 
teju\_jagua & 37 & 520 & 3.8 \\ 
double\_conversion & 75 & 1100 & 3.7 \\ 
swiftDtoa & 41 & 660 & 4.3 \\ 
yy\_double & 28 & 490 & 4.6 \\ 
std::to\_chars & 46 & 860 & 5.0 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 2400 & 5.0 \\ 
fmt\_format & 54 & 900 & 4.4 \\ 
grisu\_exact & 33 & 490 & 3.8 \\ 
schubfach & 28 & 460 & 4.3 \\ 
dragonbox & 26 & 390 & 3.8 \\ 
ryu & 31 & 520 & 4.4 \\ 
teju\_jagua & 31 & 450 & 3.8 \\ 
double\_conversion & 65 & 910 & 3.7 \\ 
swiftDtoa & 31 & 490 & 4.1 \\ 
std::to\_chars & 40 & 680 & 4.5 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 110 & 2300 & 5.2 \\ 
netlib & 280 & 3900 & 3.8 \\ 
fmt\_format & 35 & 610 & 4.6 \\ 
grisu3 & 19 & 310 & 4.3 \\ 
grisu\_exact & 23 & 390 & 4.5 \\ 
schubfach & 15 & 270 & 4.7 \\ 
dragonbox & 14 & 270 & 5.1 \\ 
ryu & 19 & 350 & 4.9 \\ 
teju\_jagua & 17 & 260 & 4.2 \\ 
double\_conversion & 42 & 630 & 4.0 \\ 
swiftDtoa & 31 & 530 & 4.4 \\ 
yy\_double & 14 & 230 & 4.2 \\ 
std::to\_chars & 27 & 520 & 5.0 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 88 & 1700 & 5.0 \\ 
fmt\_format & 30 & 530 & 4.6 \\ 
grisu\_exact & 22 & 330 & 3.9 \\ 
schubfach & 15 & 240 & 4.2 \\ 
dragonbox & 13 & 220 & 4.3 \\ 
ryu & 22 & 400 & 4.7 \\ 
teju\_jagua & 16 & 240 & 4.0 \\ 
double\_conversion & 44 & 640 & 3.9 \\ 
swiftDtoa & 20 & 310 & 4.0 \\ 
std::to\_chars & 32 & 560 & 4.6 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 260 & 4900 & 5.0 \\ 
netlib & 770 & 12000 & 4.2 \\ 
fmt\_format & 43 & 590 & 3.6 \\ 
grisu3 & 43 & 520 & 3.2 \\ 
grisu\_exact & 28 & 380 & 3.6 \\ 
schubfach & 28 & 340 & 3.2 \\ 
dragonbox & 21 & 250 & 3.2 \\ 
ryu & 26 & 400 & 4.1 \\ 
teju\_jagua & 27 & 320 & 3.0 \\ 
double\_conversion & 63 & 830 & 3.5 \\ 
swiftDtoa & 36 & 470 & 3.4 \\ 
yy\_double & 25 & 280 & 3.0 \\ 
std::to\_chars & 38 & 640 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c7i.metal-24xl/Intel_R__Xeon_R__Platinum_8488C_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 140 & 2300 & 4.3 \\ 
fmt\_format & 34 & 460 & 3.5 \\ 
grisu\_exact & 27 & 290 & 2.8 \\ 
schubfach & 23 & 250 & 2.9 \\ 
dragonbox & 17 & 180 & 2.7 \\ 
ryu & 24 & 320 & 3.4 \\ 
teju\_jagua & 25 & 240 & 2.5 \\ 
double\_conversion & 53 & 680 & 3.4 \\ 
swiftDtoa & 28 & 290 & 2.7 \\ 
std::to\_chars & 34 & 460 & 3.6 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_clang++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 220 & 3300 & 5.3 \\ 
netlib & 1800 & 12000 & 2.4 \\ 
fmt\_format & 68 & 830 & 4.4 \\ 
grisu3 & 52 & 650 & 4.4 \\ 
grisu\_exact & 44 & 550 & 4.4 \\ 
schubfach & 41 & 520 & 4.6 \\ 
dragonbox & 33 & 450 & 5.0 \\ 
ryu & 40 & 540 & 4.8 \\ 
teju\_jagua & 41 & 490 & 4.3 \\ 
double\_conversion & 93 & 1100 & 4.2 \\ 
swiftDtoa & 42 & 560 & 4.8 \\ 
yy\_double & 32 & 430 & 4.8 \\ 
std::to\_chars & 54 & 800 & 5.4 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_clang++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 1800 & 5.1 \\ 
fmt\_format & 54 & 730 & 4.8 \\ 
grisu\_exact & 37 & 460 & 4.5 \\ 
schubfach & 32 & 450 & 5.1 \\ 
dragonbox & 30 & 400 & 4.8 \\ 
ryu & 32 & 460 & 5.1 \\ 
teju\_jagua & 36 & 450 & 4.4 \\ 
double\_conversion & 80 & 950 & 4.2 \\ 
swiftDtoa & 34 & 490 & 5.1 \\ 
std::to\_chars & 45 & 640 & 5.1 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_clang++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 110 & 1600 & 5.4 \\ 
netlib & 660 & 4000 & 2.2 \\ 
fmt\_format & 44 & 530 & 4.3 \\ 
grisu3 & 21 & 290 & 4.9 \\ 
grisu\_exact & 27 & 340 & 4.6 \\ 
schubfach & 16 & 230 & 5.3 \\ 
dragonbox & 19 & 250 & 4.8 \\ 
ryu & 21 & 290 & 4.8 \\ 
teju\_jagua & 17 & 230 & 4.7 \\ 
double\_conversion & 55 & 640 & 4.2 \\ 
swiftDtoa & 31 & 400 & 4.5 \\ 
yy\_double & 13 & 170 & 4.9 \\ 
std::to\_chars & 31 & 480 & 5.5 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_clang++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 81 & 1200 & 5.4 \\ 
fmt\_format & 33 & 450 & 4.9 \\ 
grisu\_exact & 21 & 270 & 4.5 \\ 
schubfach & 15 & 210 & 4.9 \\ 
dragonbox & 16 & 200 & 4.7 \\ 
ryu & 25 & 320 & 4.6 \\ 
teju\_jagua & 18 & 220 & 4.4 \\ 
double\_conversion & 55 & 650 & 4.2 \\ 
swiftDtoa & 22 & 290 & 4.7 \\ 
std::to\_chars & 34 & 500 & 5.3 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_clang++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 230 & 3400 & 5.3 \\ 
netlib & 2000 & 13000 & 2.3 \\ 
fmt\_format & 48 & 490 & 3.7 \\ 
grisu3 & 45 & 470 & 3.8 \\ 
grisu\_exact & 32 & 330 & 3.7 \\ 
schubfach & 28 & 290 & 3.6 \\ 
dragonbox & 23 & 230 & 3.6 \\ 
ryu & 28 & 310 & 4.0 \\ 
teju\_jagua & 28 & 260 & 3.3 \\ 
double\_conversion & 77 & 870 & 4.0 \\ 
swiftDtoa & 34 & 360 & 3.8 \\ 
yy\_double & 18 & 200 & 3.9 \\ 
std::to\_chars & 40 & 570 & 5.0 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_clang++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 120 & 1700 & 5.0 \\ 
fmt\_format & 33 & 390 & 4.2 \\ 
grisu\_exact & 28 & 240 & 3.1 \\ 
schubfach & 23 & 220 & 3.5 \\ 
dragonbox & 19 & 170 & 3.2 \\ 
ryu & 24 & 240 & 3.7 \\ 
teju\_jagua & 27 & 220 & 3.0 \\ 
double\_conversion & 63 & 710 & 4.0 \\ 
swiftDtoa & 29 & 300 & 3.6 \\ 
std::to\_chars & 34 & 410 & 4.4 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_g++_canada_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 230 & 3500 & 5.6 \\ 
netlib & 1800 & 12000 & 2.4 \\ 
fmt\_format & 84 & 1200 & 5.1 \\ 
grisu3 & 51 & 690 & 4.8 \\ 
grisu\_exact & 45 & 610 & 4.8 \\ 
schubfach & 38 & 540 & 5.0 \\ 
dragonbox & 33 & 460 & 5.0 \\ 
ryu & 42 & 600 & 5.2 \\ 
teju\_jagua & 41 & 530 & 4.6 \\ 
double\_conversion & 84 & 1000 & 4.4 \\ 
swiftDtoa & 42 & 560 & 4.8 \\ 
yy\_double & 34 & 480 & 5.1 \\ 
std::to\_chars & 55 & 810 & 5.2 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_g++_canada_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 1900 & 5.3 \\ 
fmt\_format & 70 & 870 & 4.5 \\ 
grisu\_exact & 37 & 500 & 4.8 \\ 
schubfach & 32 & 470 & 5.2 \\ 
dragonbox & 30 & 410 & 4.9 \\ 
ryu & 34 & 500 & 5.2 \\ 
teju\_jagua & 35 & 460 & 4.7 \\ 
double\_conversion & 72 & 890 & 4.4 \\ 
swiftDtoa & 36 & 490 & 4.9 \\ 
std::to\_chars & 46 & 640 & 5.0 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_g++_mesh_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 110 & 1700 & 5.5 \\ 
netlib & 660 & 4000 & 2.2 \\ 
fmt\_format & 49 & 610 & 4.4 \\ 
grisu3 & 21 & 310 & 5.2 \\ 
grisu\_exact & 28 & 400 & 5.1 \\ 
schubfach & 15 & 250 & 5.8 \\ 
dragonbox & 17 & 250 & 5.2 \\ 
ryu & 21 & 320 & 5.4 \\ 
teju\_jagua & 17 & 250 & 5.0 \\ 
double\_conversion & 46 & 600 & 4.6 \\ 
swiftDtoa & 34 & 410 & 4.3 \\ 
yy\_double & 17 & 210 & 4.5 \\ 
std::to\_chars & 32 & 480 & 5.4 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_g++_mesh_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 87 & 1300 & 5.5 \\ 
fmt\_format & 47 & 520 & 4.0 \\ 
grisu\_exact & 22 & 310 & 5.2 \\ 
schubfach & 14 & 220 & 5.5 \\ 
dragonbox & 15 & 200 & 5.0 \\ 
ryu & 25 & 350 & 5.0 \\ 
teju\_jagua & 17 & 220 & 4.8 \\ 
double\_conversion & 47 & 610 & 4.6 \\ 
swiftDtoa & 22 & 290 & 4.7 \\ 
std::to\_chars & 34 & 500 & 5.2 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_g++_uniform_01_none.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 240 & 3700 & 5.4 \\ 
netlib & 2000 & 13000 & 2.3 \\ 
fmt\_format & 52 & 590 & 4.0 \\ 
grisu3 & 45 & 500 & 4.0 \\ 
grisu\_exact & 33 & 380 & 4.1 \\ 
schubfach & 28 & 300 & 3.9 \\ 
dragonbox & 23 & 230 & 3.6 \\ 
ryu & 29 & 360 & 4.4 \\ 
teju\_jagua & 29 & 290 & 3.7 \\ 
double\_conversion & 68 & 780 & 4.1 \\ 
swiftDtoa & 35 & 360 & 3.7 \\ 
yy\_double & 25 & 240 & 3.5 \\ 
std::to\_chars & 41 & 570 & 5.0 \\ 
\bottomrule
\end{tabular}


==> results/c8g.medium/Neoverse-V2_g++_uniform_01_s.tex <==

\begin{tabular}{lccc}
\toprule
\textbf{Name} & \textbf{ns/f} & \textbf{instructions/float} & \textbf{instructions/cycle} \\
\midrule
dragon4 & 130 & 1800 & 5.1 \\ 
fmt\_format & 44 & 460 & 3.7 \\ 
grisu\_exact & 27 & 280 & 3.6 \\ 
schubfach & 21 & 230 & 3.9 \\ 
dragonbox & 19 & 170 & 3.2 \\ 
ryu & 25 & 270 & 3.9 \\ 
teju\_jagua & 26 & 230 & 3.1 \\ 
double\_conversion & 55 & 650 & 4.2 \\ 
swiftDtoa & 30 & 290 & 3.5 \\ 
std::to\_chars & 34 & 410 & 4.3 \\ 
\bottomrule
\end{tabular}

